Finite-Sum Optimization: A New Perspective for Convergence to a Global Solution

Deep neural networks (DNNs) have shown great success in many machine learning tasks. Their training is challenging since the loss surface of the network architecture is generally non-convex, or even non-smooth. How and under what assumptions is guaranteed convergence to a \textit{global} minimum possible? We propose a reformulation of the minimization problem allowing for a new recursive algorithmic framework. By using bounded style assumptions, we prove convergence to an $\varepsilon$-(global) minimum using $\mathcal{\tilde{O}}(1/\varepsilon^3)$ gradient computations. Our theoretical foundation motivates further study, implementation, and optimization of the new algorithmic framework and further investigation of its non-standard bounded style assumptions. This new direction broadens our understanding of why and under what circumstances training of a DNN converges to a global minimum.

==> refs.tex <==
\begin{thebibliography}{42}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Abadi et al(2015)]{tensorflow2015-whitepaper}
M.~Abadi {\emph{et al}}.
\newblock {TensorFlow}: Large-scale machine learning on heterogeneous systems,
  2015.
\newblock URL \url{https://www.tensorflow.org/}.
\newblock Software available from tensorflow.org.

\bibitem[Bertsekas(2011)]{Bertsekas2011}
D.P. Bertsekas.
\newblock Incremental proximal methods for large scale convex optimization.
\newblock \emph{Math. Program.}, 129\penalty0 (2):\penalty0 163--195, 2011.

\bibitem[Bottou(2009)]{bottou2009curiously}
L.~Bottou.
\newblock Curiously fast convergence of some stochastic gradient descent
  algorithms.
\newblock 2009.

\bibitem[Bottou(2012)]{bottou2012stochastic}
L.~Bottou.
\newblock Stochastic gradient descent tricks.
\newblock In \emph{Neural networks: Tricks of the trade}, pages 421--436.
  Springer, 2012.

\bibitem[Bottou et~al.(2018)Bottou, Curtis, and Nocedal]{Bottou2018}
L.~Bottou, F.~E. Curtis, and J.~Nocedal.
\newblock {O}ptimization {M}ethods for {L}arge-{S}cale {M}achine {L}earning.
\newblock \emph{SIAM Rev.}, 60\penalty0 (2):\penalty0 223--311, 2018.

\bibitem[Chang and Lin(2011)]{LIBSVM}
Chih-Chung Chang and Chih-Jen Lin.
\newblock {LIBSVM}: A library for support vector machines.
\newblock \emph{ACM Transactions on Intelligent Systems and Technology},
  2:\penalty0 27:1--27:27, 2011.
\newblock Software available at \url{http://www.csie.ntu.edu.tw/~cjlin/libsvm}.

\bibitem[Chen et~al.(2018)Chen, Liu, Sun, and Hong]{chen2018convergence}
X.~Chen, S.~Liu, R.~Sun, and M.~Hong.
\newblock On the convergence of a class of adam-type algorithms for non-convex
  optimization.
\newblock \emph{ICLR}, 2018.

\bibitem[Defazio et~al.(2014)Defazio, Bach, and Lacoste-Julien]{SAGA}
Aaron Defazio, Francis Bach, and Simon Lacoste-Julien.
\newblock Saga: A fast incremental gradient method with support for
  non-strongly convex composite objectives.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  1646--1654, 2014.

\bibitem[Dozat(2016)]{dozat2016incorporating}
T.~Dozat.
\newblock Incorporating nesterov momentum into {ADAM}.
\newblock \emph{ICLRWorkshop}, 1:\penalty0 2013–--2016, 2016.

\bibitem[Duchi et~al.(2011)Duchi, Hazan, and Singer]{AdaGrad}
John Duchi, Elad Hazan, and Yoram Singer.
\newblock Adaptive subgradient methods for online learning and stochastic
  optimization.
\newblock \emph{Journal of Machine Learning Research}, 12:\penalty0 2121--2159,
  2011.

\bibitem[Ghadimi and Lan(2013)]{ghadimi2013stochastic}
S.~Ghadimi and G.~Lan.
\newblock Stochastic first-and zeroth-order methods for nonconvex stochastic
  programming.
\newblock \emph{SIAM J. Optim.}, 23\penalty0 (4):\penalty0 2341--2368, 2013.

\bibitem[G{\"u}rb{\"u}zbalaban et~al.(2015)G{\"u}rb{\"u}zbalaban, Ozdaglar, and
  Parrilo]{gurbuzbalaban2015random}
Mert G{\"u}rb{\"u}zbalaban, Asu Ozdaglar, and Pablo Parrilo.
\newblock Why random reshuffling beats stochastic gradient descent.
\newblock \emph{arXiv preprint arXiv:1510.08560}, 2015.

\bibitem[HaoChen and Sra(2018)]{haochen2018random}
Jeffery~Z HaoChen and Suvrit Sra.
\newblock Random shuffling beats sgd after finite epochs.
\newblock \emph{arXiv preprint arXiv:1806.10077}, 2018.

\bibitem[Johnson and Zhang(2013)]{SVRG}
Rie Johnson and Tong Zhang.
\newblock Accelerating stochastic gradient descent using predictive variance
  reduction.
\newblock In \emph{NIPS}, pages 315--323, 2013.

\bibitem[Kingma and Ba(2014)]{Kingma2014}
D.~P. Kingma and J.~Ba.
\newblock {ADAM}: {A} {M}ethod for {S}tochastic {O}ptimization.
\newblock \emph{Proceedings of the 3rd International Conference on Learning
  Representations (ICLR)}, abs/1412.6980, 2014.

\bibitem[Krizhevsky and Hinton(2009)]{CIFAR10}
Alex Krizhevsky and Geoffrey Hinton.
\newblock Learning multiple layers of features from tiny images.
\newblock Technical report, Citeseer, 2009.

\bibitem[Le~Roux et~al.(2012)Le~Roux, Schmidt, and Bach]{SAG}
Nicolas Le~Roux, Mark Schmidt, and Francis Bach.
\newblock A stochastic gradient method with an exponential convergence rate for
  finite training sets.
\newblock In \emph{NIPS}, pages 2663--2671, 2012.

\bibitem[LeCun et~al.(1998)LeCun, Bottou, Bengio, and Haffner]{MNIST}
Yann LeCun, L{\'e}on Bottou, Yoshua Bengio, and Patrick Haffner.
\newblock Gradient-based learning applied to document recognition.
\newblock \emph{Proceedings of the IEEE}, 86\penalty0 (11):\penalty0
  2278--2324, 1998.

\bibitem[Li et~al.(2020)Li, Zhuang, and Orabona]{li2020exponential}
L.~Li, Z.~Zhuang, and F.~Orabona.
\newblock Exponential step sizes for non-convex optimization.
\newblock \emph{arXiv preprint arXiv:2002.05273}, 2020.

\bibitem[Li et~al.(2019)Li, Zhu, So, and Lee]{li2019incremental}
X.~Li, Z.~Zhu, A.~So, and J.~D. Lee.
\newblock Incremental methods for weakly convex optimization.
\newblock \emph{arXiv preprint arXiv:1907.11687}, 2019.

\bibitem[Loshchilov and Hutter(2017)]{loshchilov10sgdr}
I.~Loshchilov and F.~Hutter.
\newblock {SGDR}: {S}tochastic gradient descent with warm restarts.
\newblock 10:\penalty0 1--16, 2017.

\bibitem[Loshchilov and Hutter(2016)]{loshchilov2016sgdr}
Ilya Loshchilov and Frank Hutter.
\newblock Sgdr: Stochastic gradient descent with warm restarts, 2016.

\bibitem[Meng et~al.(2019)Meng, Chen, Wang, Ma, and Liu]{meng2019convergence}
Q.~Meng, W.~Chen, Y.~Wang, Z.-M. Ma, and T.-Y. Liu.
\newblock Convergence analysis of distributed stochastic gradient descent with
  shuffling.
\newblock \emph{Neurocomputing}, 337:\penalty0 46--57, 2019.

\bibitem[Mishchenko et~al.(2020)Mishchenko, Khaled, and
  Richt{\'a}rik]{mishchenko2020random}
K.~Mishchenko, A.~Khaled, and P.~Richt{\'a}rik.
\newblock Random reshuffling: {S}imple analysis with vast improvements.
\newblock \emph{arXiv preprint arXiv:2006.05988}, 2020.

\bibitem[Nagaraj et~al.(2019)Nagaraj, Jain, and Netrapalli]{nagaraj2019sgd}
Dheeraj Nagaraj, Prateek Jain, and Praneeth Netrapalli.
\newblock Sgd without replacement: Sharper rates for general smooth convex
  functions.
\newblock In \emph{International Conference on Machine Learning}, pages
  4703--4711, 2019.

\bibitem[Nedi{\'c} and Bertsekas(2001)]{nedic2001convergence}
A.~Nedi{\'c} and D.~Bertsekas.
\newblock Convergence rate of incremental subgradient algorithms.
\newblock In \emph{Stochastic optimization: algorithms and applications}, pages
  223--264. Springer, 2001.

\bibitem[Nedic and Bertsekas(2001)]{nedic2001incremental}
A.~Nedic and D.~P. Bertsekas.
\newblock Incremental subgradient methods for nondifferentiable optimization.
\newblock \emph{SIAM J. on Optim.}, 12\penalty0 (1):\penalty0 109--138, 2001.

\bibitem[Nesterov(1983)]{Nesterov1983}
Y.~Nesterov.
\newblock A method for unconstrained convex minimization problem with the rate
  of convergence $\mathcal{O}(1/k^2)$.
\newblock \emph{Doklady AN SSSR}, 269:\penalty0 543--547, 1983.
\newblock Translated as Soviet Math. Dokl.

\bibitem[Nesterov(2004)]{Nesterov2004}
Y.~Nesterov.
\newblock \emph{{I}ntroductory lectures on convex optimization: {A} basic
  course}, volume~87 of \emph{Applied Optimization}.
\newblock Kluwer Academic Publishers, 2004.

\bibitem[Nguyen et~al.(2017)Nguyen, Liu, Scheinberg, and
  Tak{\'a}{\v{c}}]{Nguyen2017sarah}
L.~M. Nguyen, J.~Liu, K.~Scheinberg, and M.~Tak{\'a}{\v{c}}.
\newblock {SARAH}: {A} novel method for machine learning problems using
  stochastic recursive gradient.
\newblock \emph{ICML}, 2017.

\bibitem[Nguyen et~al.(2020)Nguyen, Tran-Dinh, Phan, Nguyen, and van
  Dijk]{nguyen2020unified}
L.~M. Nguyen, Q.~Tran-Dinh, D.~T. Phan, P.~H. Nguyen, and M.~van Dijk.
\newblock A unified convergence analysis for shuffling-type gradient methods.
\newblock \emph{arXiv preprint arXiv:2002.08246}, 2020.

\bibitem[Nguyen et~al.(2018)Nguyen, Nguyen, van Dijk, Richtarik, Scheinberg,
  and Takac]{Nguyen2018_sgdhogwild}
Lam Nguyen, Phuong~Ha Nguyen, Marten van Dijk, Peter Richtarik, Katya
  Scheinberg, and Martin Takac.
\newblock {SGD} and {H}ogwild! convergence without the bounded gradients
  assumption.
\newblock In \emph{Proceedings of the 35th International Conference on Machine
  Learning-Volume 80}, pages 3747--3755, 2018.
  
\bibitem[Nguyen et~al.(2019{\natexlab{a}})Nguyen, Nguyen, Richt{{\'a}}rik,
  Scheinberg, Tak{{\'a}}{\v{c}}, and van Dijk]{nguyen2019newaspect}
Lam~M. Nguyen, Phuong~Ha Nguyen, Peter Richt{{\'a}}rik, Katya Scheinberg,
  Martin Tak{{\'a}}{\v{c}}, and Marten van Dijk.
\newblock New convergence aspects of stochastic gradient algorithms.
\newblock \emph{Journal of Machine Learning Research}, 20\penalty0
  (176):\penalty0 1--49, 2019{\natexlab{a}}.

\bibitem[Paszke et al (2019)]{pytorch}
A.~Paszke {\emph{et al}}.
\newblock Pytorch: An imperative style, high-performance deep learning library.
\newblock In \emph{Advances in Neural Information Processing Systems 32}, pages
  8024--8035. Curran Associates, Inc., 2019.

\bibitem[Pham et~al.(2020)Pham, Nguyen, Phan, and Tran-Dinh]{Pham2019}
N.~H. Pham, L.~M. Nguyen, D.~T. Phan, and Q.~Tran-Dinh.
\newblock {ProxSARAH}: {A}n efficient algorithmic framework for stochastic
  composite nonconvex optimization.
\newblock \emph{J. Mach. Learn. Res.}, 2020.

\bibitem[Polyak(1964)]{polyak1964some}
B.~T. Polyak.
\newblock Some methods of speeding up the convergence of iteration methods.
\newblock \emph{USSR Computational Mathematics and Mathematical Physics},
  4\penalty0 (5):\penalty0 1--17, 1964.

\bibitem[Rajput et~al.(2020)Rajput, Gupta, and
  Papailiopoulos]{rajput2020closing}
S.~Rajput, A.~Gupta, and D.~Papailiopoulos.
\newblock Closing the convergence gap of {SGD} without replacement.
\newblock \emph{arXiv preprint arXiv:2002.10400}, 2020.

\bibitem[Reddi et~al.(2016)Reddi, Hefny, Sra, P{\'{o}}czos, and
  Smola]{Reddi2016a}
Sashank~J. Reddi, Ahmed Hefny, Suvrit Sra, Barnab{\'{a}}s P{\'{o}}czos, and
  Alexander~J. Smola.
\newblock Stochastic variance reduction for nonconvex optimization.
\newblock In \emph{ICML}, pages 314--323, 2016.

\bibitem[Robbins and Monro(1951)]{RM1951}
Herbert Robbins and Sutton Monro.
\newblock A stochastic approximation method.
\newblock \emph{The Annals of Mathematical Statistics}, 22\penalty0
  (3):\penalty0 400--407, 1951.

\bibitem[Ruder(2017)]{ruder2017overview}
Sebastian Ruder.
\newblock An overview of gradient descent optimization algorithms, 2017.

\bibitem[Safran and Shamir(2018)]{Safran2019HowGoodSGDShuffling}
I.~Safran and O.~Shamir.
\newblock How good is {SGD} with random shuffling?
\newblock \emph{arXiv preprint arXiv:1908.00045}, 2018.

\bibitem[Shamir(2016)]{shamir2016without}
O.~Shamir.
\newblock Without-replacement sampling for stochastic gradient methods.
\newblock In \emph{Advances in neural information processing systems}, pages
  46--54, 2016.

\bibitem[Smith(2017)]{smith2017cyclical}
L.~N. Smith.
\newblock Cyclical learning rates for training neural networks.
\newblock In \emph{2017 IEEE Winter Conference on Applications of Computer
  Vision (WACV)}, pages 464--472. IEEE, 2017.

\bibitem[Smith(2015)]{smith2015cyclical}
Leslie~N. Smith.
\newblock Cyclical learning rates for training neural networks, 2015.

\bibitem[Tran-Dinh et~al.(2019)Tran-Dinh, Pham, Phan, and
  Nguyen]{Tran-Dinh2019a}
Q.~Tran-Dinh, N.~H. Pham, D.~T. Phan, and L.~M. Nguyen.
\newblock A hybrid stochastic optimization framework for stochastic composite
  nonconvex optimization.
\newblock \emph{Preprint: UNC-STOR 07.10.2019}, 2019.

\bibitem[Wang et~al.(2020)Wang, Nguyen, Bertozzi, Baraniuk, and
  Osher]{wang2020scheduled}
B.~Wang, T.~M. Nguyen, A.~L. Bertozzi, R.~G. Baraniuk, and S.~J. Osher.
\newblock Scheduled restart momentum for accelerated stochastic gradient
  descent.
\newblock \emph{arXiv preprint arXiv:2002.10583}, 2020.

\bibitem[Xiao et~al.(2017)Xiao, Rasul, and Vollgraf]{xiao2017fashion}
Han Xiao, Kashif Rasul, and Roland Vollgraf.
\newblock Fashion-mnist: a novel image dataset for benchmarking machine
  learning algorithms.
\newblock \emph{arXiv preprint arXiv:1708.07747}, 2017.

\bibitem[Ying et~al.(2017)Ying, Yuan, and Sayed]{ying2017convergence}
B.~Ying, K.~Yuan, and A.~H. Sayed.
\newblock Convergence of variance-reduced stochastic learning under random
  reshuffling.
\newblock \emph{arXiv preprint arXiv:1708.01383}, 2\penalty0 (3):\penalty0 6,
  2017.

\end{thebibliography}


==> sections/ethics.tex <==
\section*{Ethics Statement}

This paper does not contain ethics concerns. 

% All ICLR participants, including authors, are required to adhere to the ICLR Code of Ethics (\url{https://iclr.cc/public/CodeOfEthics}). All authors of submitted papers are required to read the Code of Ethics, adhere to it, and explicitly acknowledge this during the submission process. The Code of Ethics applies to all conference participation, including paper submission, reviewing, and paper discussion. 

% As part of the review process, reviewers will be encouraged to raise potential violations of the ICLR Code of Ethics. If authors feel that their paper submission raises questions regarding the Code of Ethics, they are encouraged to discuss any potential issues as part of their submission. This discussion is not counted against the maximum page limit of the paper and should be included as a separate section.

% Authors who encounter potential violations of the Code of Ethics, e.g., as part of the review or public discussion, should raise these issues in a private message to their paper’s Area Chair through the open review interface.

% Authors are encouraged to include an Ethics Statement to address potential concerns where appropriate, topics include but not limited to discrimination /bias / fairness concerns, inappropriate potential applications \& impact, privacy and security issues, legal compliance, research Integrity Issues, responsible research practice (e.g., IRB, documentation, research ethics). 

% Authors are encouraged to include a paragraph of Ethics Statement (at the end of the main text before references) to address potential concerns where appropriate, topics include, but are not limited to, studies that involve human subjects, practices to data set releases, potentially harmful insights, methodologies and applications, potential conflicts of interest and sponsorship, discrimination/bias/fairness concerns, privacy and security issues, legal compliance, and research integrity issues. The optional ethic statement will not count toward the page limit. 

==> sections/experiments.tex <==
\section{Numerical Experiments}\label{sec_experiments}


==> sections/old_theory.tex <==
\subsection{OLD ALG}

For each iteration $t$, we find a search direction $v^{(t)}$ which is sufficiently close to the optimal solution $v_{*\ \text{reg}}^{(t)}$:
% \begin{align*}
%      \Psi(v^{(t)}) - \Psi(v_{*\ \text{reg}}^{(t)}) \leq \varepsilon^2, \tagthis \label{criteria_eps_sol.2}
% \end{align*}
\begin{align*}
     \| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2 \leq \delta, \tagthis \label{criteria_eps_sol.2}
\end{align*}
for some $\delta > 0$.
% Since function $\Psi$ is $\varepsilon^2$-strongly convex, we have, for $\forall v \in \mathbb{R}^d$, 
% \begin{align*}
%     \Psi(v) - \Psi(v_*) \geq \frac{\varepsilon^2}{2} \| v - v_{*\ \text{reg}}^{(t)} \|^2, \tagthis \label{eq_strongly_convex_01.2}
% \end{align*}
% where $v_{*\ \text{reg}}^{(t)}$ is the optimal solution of $\Psi$. 
% Hence, by using $\frac{1}{2}\| a \|^2 - \| b \|^2 \leq \| a - b \|^2$, we have
% \begin{align*}
%     \| v \|^2 \leq \frac{4}{\varepsilon^2} [\Psi(v) - \Psi(v_*)] + 2 \| v_* \|^2. \tagthis \label{eq_strongly_convex_02.2}
% \end{align*}
Our Algorithm \ref{alg_GD_solved.2} is described as follows.

\renewcommand{\thealgorithm}{2}
\begin{algorithm}[hpt!]
   \caption{Solve the regularized problem using Gradient Descent}
   \label{alg_GD_solved.2}
\begin{algorithmic}
   \STATE {\bfseries Initialization:} Choose an initial point $w^{(0)}\in\R^d$ % tolerance $\varepsilon > 0$ 
   and some constant $\delta > 0$;
   \FOR{$t=0,1,\cdots,T-1 $}
   \STATE Use Gradient Descent algorithm to solve Problem \peqref{opt_prob_L2} and find a solution $v^{(t)}$ that satisfies 
   $$\| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2 \leq \delta$$
   \STATE Update $w^{(t+1)} = w^{(t)} - \eta^{(t)} v^{(t)}$
   \ENDFOR
%   \STATE\textbf{Output:} 
% Choose $\hat{w}_T \in \{ w^{(0)},\cdots,w^{(T-1)}\}$ uniformly at random.
\end{algorithmic}
\end{algorithm} 




We will need the following assumption.
%====================================================================================
\begin{ass}\label{ass_bounded_hessian.2}
Let $H_i^{(t)}$ be the Jacobian matrix defined in Lemma~\ref{lem_approx_h}.
For $i = 1,\dots,n$ and $t \geq 0$, we assume that
\begin{align*}
    \| H_i^{(t)} \| \leq H, \tagthis \label{eq_ass_bounded_hessian.2}
\end{align*}
for some $H > 0$. 
\end{ass}

\begin{thm}\label{thm_main_result_GD_solved.2}
% Suppose that Assumptions ... hold and Assumption~\ref{ass_diff_optimal_eps} holds with $\delta = P \varepsilon$ for some $P > 0$ and $\varepsilon > 0$. 
Let $w^{(t)}$ be generated by Algorithm \ref{alg_GD_solved.2} where $v^{(t)}$ satisfies \peqref{criteria_eps_sol.2}. Suppose that Assumptions \ref{ass_approx_h}, \ref{ass_solve_v} %, \ref{ass_diff_optimal_eps} 
and \ref{ass_bounded_hessian.2} hold. Consider $\eta^{(t)} = D{\varepsilon}$ for some $D > 0$ and $\varepsilon > 0$ and the learning rate satisfies:
\begin{align*}
    \alpha_i^{(t)} = ( 1 + \varepsilon ) \alpha_i^{(t-1)} = ( 1 + \varepsilon )^t \alpha_i^{(0)}, \ t = 1,\dots,T  %\tagthis \label{learning_rate_power}
\end{align*}
for $\varepsilon > 0$ with $T = \frac{\beta}{\varepsilon}$ and $\alpha_i^{(0)} = \frac{\alpha}{e^{\beta} L_{\phi}}$ for some constant $\beta > 0$, $\alpha \in (0, \frac{1}{4})$.

We have
\allowdisplaybreaks
\begin{align*}
    \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] & \leq  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon \\% + P \varepsilon \\
    & \quad + \frac{e^{\beta} L_{\phi}(4\varepsilon+3)}{2\alpha( 1 - 4 \alpha)}  \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2 + 2+ V\right] \cdot \varepsilon.  \tagthis \label{eq_thm_main_result_GD_solved_new.2}
\end{align*}

% \lam{Let us choose $\varepsilon \leq 1$ so that we can convert to $\frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] \leq N \varepsilon = \hat{\varepsilon}$ and choose new $\hat{\varepsilon}$ to bring $N$ to $\Ocal$. }

\end{thm}


Proof of Theorem 1 is in Appendix \ref{sec_proofs_GD_solved.2}.


\begin{cor}\label{cor_thm_main_result_GD_solved_new.2}
Suppose that the conditions in Theorem~\ref{thm_main_result_GD_solved.2} hold with $\eta^{(t)} = \frac{D}{N} \hat{\varepsilon}$ for some $D > 0$ and $0 < \hat{\varepsilon} \leq N$, where 
\begin{align*}
    N = \tfrac{e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha \beta}  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 + \tfrac{7 e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2)^2 + 2+ V\right]. 
\end{align*} 
Then, the total complexity to guarantee $\min_{1 \leq t \leq T} [ F (w^{(t)}) - F_* ] \leq \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] \leq \hat{\varepsilon}$
% \begin{align*}
%     \min_{1 \leq t \leq T} [ F (w^{(t)}) - F_* ] \leq \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] \leq \hat{\varepsilon}
% \end{align*}
is $\mathcal{O}\left(\frac{n N \beta (D^2 H^2 + 1)}{\hat{\varepsilon}} \log(1/\delta) \right)$. 
\end{cor}

% \lam{We will need to write the exact number of accuracy and gradient evaluations without using big O}

\begin{proof} \textcolor{blue}{We may bring this proof to appendix.}
For each iteration $t \geq 0$, we need to find $v^{(t)}$ satisfying the following criteria: 
%Notice that, for strongly convex problem we can find $v^{(t)}$ so that, for $t \geq 0$,
% \begin{align*}
%      \Psi(v^{(t)}) - \Psi(v_{*\ \text{reg}}^{(t)}) \leq \varepsilon^2, 
% \end{align*}
\begin{align*}
     \| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2 \leq \delta, 
\end{align*}
for some $\delta > 0$. Using Gradient Descent we need $\mathcal{O}(n \frac{L}{\mu} \log(1/\delta))$ number of gradient evaluations \citep{nesterov2004}, where $L$ and $\mu = \varepsilon^2$ are the smooth and strongly convex constants, respectively, of $\Psi$. Let 
\begin{align*}
    \psi_i (v) = \frac{1}{2} \| H_i^{(t)} \eta^{(t)} v - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2, \ i = 1,\dots,n. \tagthis \label{eq_func_v.2}
\end{align*}
Then, for any $v \in \mathbb{R}^c$
\begin{align*}
    \nabla_v \psi_i (v) = \eta^{(t)} H_i^{(t)}{^\top} [ H_i^{(t)} \eta^{(t)} v - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) ], \ i = 1,\dots,n. \tagthis \label{eq_grad_v.2}
\end{align*}
% and
% \begin{align*}
%     H_i^{(t)}{^\top} H_i^{(t)} = \left(  \sum_{j=1}^{c} \frac{\partial h(w^{(t)} ; i)_j}{\partial w_{m_r}} \cdot \frac{\partial h(w^{(t)} ; i)_j}{\partial w_{m_c}} \right) \ , \ m_r = 1,\dots,d, \ m_c = 1,\dots,d. \tagthis \label{matrix_H_H.2}
% \end{align*}
Consider $\eta^{(t)} = D {\varepsilon}$ for some $D > 0$ and $\varepsilon > 0$, we have for $i = 1,\dots,n$ and $t \geq 0$
\begin{align*}
    \| \nabla^2_v \psi_i ( v ) \| = (\eta^{(t)})^2 \| H_i^{(t)}{^\top} H_i^{(t)} \| \leq (\eta^{(t)})^2 \| H_i^{(t)} \| \cdot \| H_i^{(t)} \| \overset{\peqref{eq_ass_bounded_hessian.2}}{\leq} D^2 \varepsilon^2 H^2. 
\end{align*}

Hence, $\| \nabla^2_v \Phi(v) \| \leq \| \nabla^2_v \psi_i ( v ) \| + \varepsilon^2 $ for any $v \in \mathbb{R}^c$ which implies that $L = D^2 \varepsilon^2 H^2 + \varepsilon^2$ (\cite{nesterov2004}) and $\frac{L}{\mu} = \frac{D^2H^2 \varepsilon^2  + \varepsilon^2}{\varepsilon^2} = D^2 H^2+1$. Therefore, the complexity to find $v^{(t)}$ for each iteration $t$ is $\mathcal{O}(n (D^2 H^2+1)\log(1/\delta))$.  

Let us choose $0 < \varepsilon \leq 1$. From \peqref{eq_thm_main_result_GD_solved_new.2}, we have
\begin{align*}
    \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] & \leq  \frac{ e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha) \alpha \beta} \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon \\% + P \varepsilon \\
    & \quad + \frac{7 e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2)^2 + 2+ V\right] \cdot \varepsilon  = N \varepsilon, 
\end{align*}
where 
\begin{align*}
    N = \tfrac{ e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha \beta}  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 + \tfrac{7 e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2)^2 + 2+ V\right]. 
\end{align*}

Let $\hat{\varepsilon} = N \varepsilon$ with $0< \hat{\varepsilon} \leq N$. Then, we need $T = \frac{N \beta}{\hat{\varepsilon}}$ for some $\beta > 0$ to guarantee $\min_{1 \leq t \leq T} [ F (w^{(t)}) - F_* ] \leq \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] \leq \hat{\varepsilon}$. Hence, the total complexity is $\mathcal{O}\left(\frac{n N \beta (D^2 H^2 + 1)}{\hat{\varepsilon}} \log(1/\delta) \right)$.
\end{proof}





%====================================================================================





% \begin{lem}\label{lem_main_result_01}
% Suppose that Assumptions ... hold. We have
% \begin{align*}
%     \| h(w^{(t+1)};i) - h_i^* \|^2 & \leq \| h(w^{(t)};i) - h_i^* \|^2 + 4 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     & \quad + 2 D \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\
%     & \quad - \frac{( 1 - 4 \alpha)  \alpha}{L_{\phi}}  [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] + 8 C^2 H^2 \varepsilon^2 + 2 \sqrt{2} D C H \varepsilon  \\
%     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 + 2 D \sqrt{c} (4 \varepsilon^2 + 4 + 2 V) G C^2 \varepsilon. \tagthis \label{eq_lem_main_result_01}
% \end{align*}
% \end{lem}

% \begin{proof}
% Note that $v^{(t)}$ is obtained from the optimization problem \peqref{opt_prob_L2} for $t \geq 0$. From \peqref{eq_002.1}, we have, for $i = 1,\dots,n$,
% \begin{align*}
%     h(w^{(t+1)};i) & = x_i^{(t+1)} = x_i^{(t)} =  h(w^{(t)} - \eta^{(t)} v^{(t)} ;i) \\
%     %
%     & = h(w^{(t)};i) - H_i^{(t)} \eta^{(t)} v^{(t)} + \epsilon_i^{(t)} \\
%     %
%     &= h(w^{(t)};i) - \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) + \epsilon_i^{(t)} \\ & \qquad - [ H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) ]. 
% \end{align*}

% Hence, we have
% \allowdisplaybreaks
% \begin{align*}
%     \| h(w^{(t+1)};i) - h_i^* \|^2
%     &= \| h(w^{(t)};i) - h_i^* - \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) + \epsilon_i^{(t)} \\ & \qquad - [ H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) ] \|^2 \\
%     %
%     &= \| h(w^{(t)};i) - h_i^* \|^2 + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     & \quad + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + \| \epsilon_i^{(t)} \|^2 \\ & \quad + \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     & \quad - 2 \langle h(w^{(t)};i) - h_i^* , \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \rangle \\ & \quad - 2 \alpha_i^{(t)} \langle  h(w^{(t)};i) - h_i^* , \nabla_x \phi_i (h(w^{(t)};i)) \rangle + 2 \langle h(w^{(t)};i) - h_i^* , \epsilon_i^{(t)} \rangle \\
%     & \quad + 2  \langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) ,  \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \rangle \\
%     & \quad - 2 \langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) , \epsilon_i^{(t)} \rangle - 2  \langle \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) , \epsilon_i^{(t)} \rangle \\
%     & \quad - 2 \langle h(w^{(t)};i) - h_i^* , H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \rangle \\
%     & \quad + 2 \langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}), H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \rangle \\
%     & \quad + 2 \langle \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)), H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \rangle \\
%     & \quad - 2 \langle \epsilon_i^{(t)}, H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \rangle \\
%     %
%     & \overset{(a)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     & \quad + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     & \quad + 2 \| h(w^{(t)};i) - h_i^* \| \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \| \\ & \quad - 2 \alpha_i^{(t)} \langle  h(w^{(t)};i) - h_i^* , \nabla_x \phi_i (h(w^{(t)};i)) \rangle + 2 \| h(w^{(t)};i) - h_i^* \| \| \epsilon_i^{(t)} \| \\
%     & \quad + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     & \quad + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 + \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + 2 \| h(w^{(t)};i) - h_i^* \| \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\
%     & \quad + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 + \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     & \quad + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2  \\
%     & \quad + \| \epsilon_i^{(t)} \|^2 + \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     %
%     & \overset{\peqref{eq_phi_convex},\peqref{eq_ass_bounded_output}}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + 4 ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     & \quad + 4 ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + 4 \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + 4 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     & \quad + 2 D \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \| + 2 D \| \epsilon_i^{(t)} \| \\ 
%     & \quad + 2 D \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\
%     & \quad - 2 \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] \\
%     %
%     & \overset{(b)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + 4 ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     & \quad + 4 \| \epsilon_i^{(t)} \|^2 + 4 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     & \quad + 2 D \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \| + 2 D \| \epsilon_i^{(t)} \| \\ 
%     & \quad + 2 D \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\
%     & \quad - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ] \\
%     %
%     & \overset{(c)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + 4 ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     & \quad + 4 \| \epsilon_i^{(t)} \|^2 + 4 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     & \quad + 2 D \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \| + 2 D \| \epsilon_i^{(t)} \| \\ 
%     & \quad + 2 D \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\
%     & \quad - \frac{( 1 - 4 \alpha)  \alpha}{L_{\phi}}  [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] \\
%     %
%     & \overset{(d)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + 4 C^2 H^2 \| v^{(t)} - v_{*\ \text{reg}}^{(t)}  \|^2 + 4 \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + 4 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 + 2 D C H  \| v^{(t)} - v_{*\ \text{reg}}^{(t)}  \| \\
%     & \quad + 2 D \| \epsilon_i^{(t)} \| + 2 D \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\ 
%     & \quad - \frac{( 1 - 4 \alpha)  \alpha}{L_{\phi}}  [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] \\
%     %
%     & \overset{(e)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + 4 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     & \quad + 2 D \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\
%     & \quad - \frac{( 1 - 4 \alpha)  \alpha}{L_{\phi}}  [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] + 8 C^2 H^2 \varepsilon^2 + 2 \sqrt{2} D C H \varepsilon  \\
%     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 + 2 D \sqrt{c} (4 \varepsilon^2 + 4 + 2 V) G C^2 \varepsilon,
% \end{align*}
% where $(a)$ follows by applying Young's inequality: $| \langle a , b \rangle | \leq \frac{\| a \|^2}{2} + \frac{\| b \|^2}{2}$ and Cauchy–Schwarz inequality $| \langle a, b \rangle | \leq \| a \| \| b \|$, $(b)$ follows by applying \peqref{eq_phi_convex_smooth} to get $\| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \leq 2 L_{\phi} [ \phi_i (h(w^{(t)};i)) - \phi_i (h_i^* ) ]$ and the fact that $\alpha_i^{(t)} \leq \frac{\alpha}{L_{\phi}}$, for some $\alpha \in (0, \frac{1}{4})$; $(c)$ follows by choosing $\alpha_i^{(t)} = \frac{\alpha}{2 L_{\phi}} \leq \frac{\alpha}{L_{\phi}}$; $(d)$ follows by using matrix vector inequality $\| H v \| \leq \| H \| \|v \| $, where $H \in \mathbb{R}^{c \times d}$ and $v \in \mathbb{R}^d$ \textbf{(NEED TO CHECK THIS since $H$ is non-square)} and Assumption~\ref{ass_bounded_hessian} in \peqref{eq_ass_bounded_hessian} and $\eta^{(t)} = C \sqrt{\varepsilon}$ for some $C > 0$ and $\varepsilon > 0$; $(e)$ follows by Lemmas~\ref{lem_bound_v} and \ref{lem_bound_epsilon}. 

% \end{proof}

% \begin{lem}\label{lem_main_result_02}
% Suppose that Assumptions ... hold. We have
% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] & \leq \frac{D L_{\phi}}{( 1 - 4 \alpha)  \alpha T} + \frac{4 ( 1 + \frac{V}{2} ) L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 + \frac{2 D L_{\phi} \sqrt{1 + \frac{V}{2}} }{( 1 - 4 \alpha)  \alpha} \varepsilon \\
%     & \quad + \frac{8 C^2 H^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha}  \varepsilon^2 + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon  \\
%     & \quad + \frac{ 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 \\
%     & \quad + \frac{ 2 D \sqrt{c} (4 \varepsilon^2 + 4 + 2 V) G C^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon. \tagthis \label{eq_lem_main_result_02}
% \end{align*}
% \end{lem}

% \begin{proof}
% Rearranging the terms in Lemma~\ref{lem_main_result_01},
% we have
% \allowdisplaybreaks
% \begin{align*}
%      \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) & \leq \frac{L_{\phi}}{( 1 - 4 \alpha)  \alpha} [  \| h(w^{(t)};i) - h_i^* \|^2  -   \| h(w^{(t+1)};i) - h_i^* \|^2  ] \\
%     & \quad + \frac{4 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     & \quad + \frac{2 D L_{\phi}}{( 1 - 4 \alpha)  \alpha} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\
%     & \quad + \frac{8 C^2 H^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha}  \varepsilon^2 + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon  \\
%     & \quad + \frac{ 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 \\
%     & \quad + \frac{ 2 D \sqrt{c} (4 \varepsilon^2 + 4 + 2 V) G C^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon
% \end{align*}

% Taking the average sum from $t = 0,\dots,T-1$, we have
% \begin{align*}
%      \frac{1}{T} \sum_{t=0}^{T-1}  [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  & \leq \frac{L_{\phi}}{( 1 - 4 \alpha)  \alpha T} \| h(w^{(0)};i) - h_i^* \|^2 \\
%     & \quad + \frac{4 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \frac{1}{T} \sum_{t=0}^{T-1} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     & \quad + \frac{2 D L_{\phi}}{( 1 - 4 \alpha)  \alpha} \frac{1}{T} \sum_{t=0}^{T-1} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\
%     & \quad + \frac{8 C^2 H^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha}  \varepsilon^2 + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon  \\
%     & \quad + \frac{ 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 \\
%     & \quad + \frac{ 2 D \sqrt{c} (4 \varepsilon^2 + 4 + 2 V) G C^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon. 
% \end{align*}
% Taking the average sum from $i = 1,\dots,n$, we have
% \begin{align*}
%     & \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  \\ & \leq \frac{L_{\phi}}{( 1 - 4 \alpha)  \alpha T} \frac{1}{n} \sum_{i=1}^n \| h(w^{(0)};i) - h_i^* \|^2 \\
%     & \quad + \frac{4 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     & \quad + \frac{2 D L_{\phi}}{( 1 - 4 \alpha)  \alpha} \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\
%     & \quad + \frac{8 C^2 H^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha}  \varepsilon^2 + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon  \\
%     & \quad + \frac{ 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 \\
%     & \quad + \frac{ 2 D \sqrt{c} (4 \varepsilon^2 + 4 + 2 V) G C^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon \\
%     & \overset{\peqref{eq_lem_stronglyconvex_prob},\peqref{eq_ass_bounded_output}}{\leq}  \frac{D L_{\phi}}{( 1 - 4 \alpha)  \alpha T} + \frac{4 ( 1 + \frac{V}{2} ) L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 + \frac{2 D L_{\phi} \sqrt{1 + \frac{V}{2}} }{( 1 - 4 \alpha)  \alpha} \varepsilon \\
%     & \quad + \frac{8 C^2 H^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha}  \varepsilon^2 + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon  \\
%     & \quad + \frac{ 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 \\
%     & \quad + \frac{ 2 D \sqrt{c} (4 \varepsilon^2 + 4 + 2 V) G C^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon,
% \end{align*}
% where the last inequality follows by Jensen's inequality \textbf{(NEED TO CHECK THIS)}
% \begin{align*}
%     \frac{1}{n} \sum_{i=1}^n \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \leq \sqrt{\frac{1}{n} \sum_{i=1}^n \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2}. 
% \end{align*}
% \end{proof}

% Note that
% \begin{align*}
%      \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  = \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ]. \tagthis \label{eq_average_phi_02}
% \end{align*}

% Using the following ``over-paramerized'' assumption
% \begin{ass}\label{ass_diff_optimal_eps}
% For some $\delta > 0$, we have
% \begin{align*}
%     \Big | F_* - \frac{1}{n} \sum_{i=1}^{n} \phi_i (h_i^* )  \Big | \leq \delta. \tagthis \label{eq_ass_diff_optimal_eps}
% \end{align*}
% \end{ass}

% \begin{thm}\label{thm_main_result_01}
% Suppose that Assumptions ... hold and Assumption~\ref{ass_diff_optimal_eps} holds with $\delta = P \varepsilon$ for some $P > 0$ and $\varepsilon > 0$. Then, we have
% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] & \leq \frac{D L_{\phi}}{( 1 - 4 \alpha)  \alpha T} + \frac{4 ( 1 + \frac{V}{2} ) L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 + \frac{2 D L_{\phi} \sqrt{1 + \frac{V}{2}} }{( 1 - 4 \alpha)  \alpha} \varepsilon \\
%     & \quad + \frac{8 C^2 H^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha}  \varepsilon^2 + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon  \\
%     & \quad + \frac{ 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 \\
%     & \quad + \frac{ 2 D \sqrt{c} (4 \varepsilon^2 + 4 + 2 V) G C^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon + P \varepsilon. \tagthis \label{eq_thm_main_result_01}
% \end{align*}
% \end{thm}

% \begin{proof}
% We have
% \allowdisplaybreaks
% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] & = \frac{1}{T} \sum_{t=0}^{T-1} \left( \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] - \left[ F_* - \frac{1}{n} \sum_{i=1}^{n} \phi_i (h_i^* )  \right] \right) \\
%     & \leq \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] \\% + P \varepsilon \\
%     % 
%     & \overset{\peqref{eq_lem_main_result_02},\peqref{eq_ass_diff_optimal_eps}}{\leq} \frac{D L_{\phi}}{( 1 - 4 \alpha)  \alpha T} + \frac{4 ( 1 + \frac{V}{2} ) L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 + \frac{2 D L_{\phi} \sqrt{1 + \frac{V}{2}} }{( 1 - 4 \alpha)  \alpha} \varepsilon \\
%     & \quad + \frac{8 C^2 H^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha}  \varepsilon^2 + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon  \\
%     & \quad + \frac{ 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon^2 \\
%     & \quad + \frac{ 2 D \sqrt{c} (4 \varepsilon^2 + 4 + 2 V) G C^2 L_{\phi}}{( 1 - 4 \alpha)  \alpha} \varepsilon + P \varepsilon. 
% \end{align*}
% \end{proof}

% \begin{cor}\label{cor_thm_main_result_01}
% Suppose that the conditions in Theorem~\ref{thm_main_result_01} hold. Then, the total complexity to guarantee
% \begin{align*}
%     \min_{0 \leq t \leq T-1} [ F (w^{(t)}) - F_* ] \leq \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] \leq \mathcal{O}(\varepsilon)
% \end{align*}
% is $\mathcal{O}\left(\frac{n (C^2 H^2 + \varepsilon^2)}{\varepsilon^3} \log(1/\varepsilon^4) \right)$. 
% \end{cor}

% \begin{proof}
% It is clear that from \peqref{eq_thm_main_result_01}, we have
% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] \leq \mathcal{O}(\varepsilon)
% \end{align*}

% after $T = \Ocal(\frac{1}{\varepsilon})$. Hence, the total complexity is $\mathcal{O}\left(\frac{n (C^2 H^2 + \varepsilon^2)}{\varepsilon^3} \log(1/\varepsilon^4) \right)$. \textbf{[It is possible to write explicitly]} 
% \end{proof}

%\subsection{New Proof}

\subsection{OLD THEORY}

% ==========================================================
% Proof for Theorem GD_solved.2
% ==========================================================

\section{Technical Proofs for Theorem \ref{thm_main_result_GD_solved.2}}\label{sec_proofs_GD_solved.2}

%\textbf{NEW ANALYSIS}



% \begin{lem}\label{lem_bound_v.2}
% For $t \geq 0$, suppose that Assumption  \ref{ass_solve_v} holds and $v^{(t)}$ satisfies \peqref{criteria_eps_sol.2}. Hence, 
% \begin{enumerate}
%     \item $\| v^{(t)} \|^2 \leq 8 + 2 V$, 
%     \item $ \| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2 \leq 2 $. 
% \end{enumerate}
% \end{lem}

% \begin{proof}
% Since function $\Psi$ is $\varepsilon^2$-strongly convex, we have, for $\forall v \in \mathbb{R}^d$, 
% \begin{align*}
%     \Psi(v) - \Psi(v_*) \geq \frac{\varepsilon^2}{2} \| v - v_{*\ \text{reg}}^{(t)} \|^2, \tagthis \label{eq_strongly_convex_01.2}
% \end{align*}
% where $v_{*\ \text{reg}}^{(t)}$ is the optimal solution of $\Psi$. Hence, by using $\frac{1}{2}\| a \|^2 - \| b \|^2 \leq \| a - b \|^2$, we have
% \begin{align*}
%     \| v \|^2 \leq \frac{4}{\varepsilon^2} [\Psi(v) - \Psi(v_{*\ \text{reg}}^{(t)})] + 2 \| v_{*\ \text{reg}}^{(t)}\|^2. \tagthis \label{eq_strongly_convex_02.2}
% \end{align*}


% 1) By \peqref{eq_strongly_convex_02.2}, we have
% \begin{align*}
%     \| v^{(t)} \|^2 \leq \frac{4}{\varepsilon^2} [\Psi(v^{(t)}) - \Psi(v_{*\ \text{reg}}^{(t)})] + 2 \| v_{*\ \text{reg}}^{(t)} \|^2 \overset{\peqref{criteria_eps_sol.2}}{\leq} 4  + 4 + 2 V,
% \end{align*}
% where the last inequality follows since $\| v_{*\ \text{reg}}^{(t)} \|^2 \leq 2+ V$ for some $V > 0$ in Lemma~\ref{lem_stronglyconvex_prob}. 

% 2) By \peqref{eq_strongly_convex_01.2}, we have
% \begin{align*}
%      \| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2 \leq \frac{2}{\varepsilon^2} [\Psi(v^{(t)}) - \Psi(v_{*\ \text{reg}}^{(t)})] \leq 2. 
% \end{align*}
% \end{proof}



\begin{lem}\label{lem_bound_v.2}
For $t \geq 0$, suppose that Assumption  \ref{ass_solve_v} holds and $v^{(t)}$ satisfies \peqref{criteria_eps_sol.2}. Then 
\begin{align*}
    \| v \|^2 \leq 2(\delta + V+2). 
\end{align*}
\end{lem}

\begin{proof} From $\| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2 \leq \delta$.
Using $\| a \|^2 \leq 2\| a - b \|^2+2 \| b \|^2 $, we have
\begin{align*}
    \| v \|^2 \leq 2\| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2  + 2 \| v_{*\ \text{reg}}^{(t)}\|^2 \overset{\peqref{criteria_eps_sol.2}}{\leq} 2\delta  + 4 + 2 V. 
\end{align*}
where the last inequality follows since $\| v_{*\ \text{reg}}^{(t)} \|^2 \leq 2+ V$ for some $V > 0$ in Lemma~\ref{lem_stronglyconvex_prob}. 


\end{proof}

\begin{lem}\label{lem_bound_epsilon.2}
Suppose that Assumptions~\ref{ass_approx_h} and \ref{ass_solve_v} hold. Consider $\eta^{(t)} = D{\varepsilon}$ for some $D > 0$ and $\varepsilon > 0$. For $i = 1,\dots,n$ and $t \geq 0$, we have
\begin{align*}
    \| \epsilon_i^{(t)} \|^2 \leq c (2+(V+\delta +2) G D^2 \varepsilon)^2\varepsilon^2  .  \tagthis \label{eq_lem_bound_epsilon.2}
\end{align*}
\end{lem}

\begin{proof}
From \peqref{eq_epsilon}, for $i = 1,\dots,n$, $j = 1,\dots,c$, and $\forall t \geq 0$, by Lemma~\ref{lem_approx_h} we have
\begin{align*}
    | \epsilon_{i,j}^{(t)} | & \leq  \frac{1}{2}(\eta^{(t)})^2 \| v^{(t)} \|^2 G + 2\varepsilon \leq \frac{1}{2}2(\delta + V+2) G D^2 \varepsilon^2 + 2\varepsilon = \varepsilon (2+(V+\delta +2) G D^2 \varepsilon) ,  
\end{align*}
where the last inequality follows by the application of Lemma~\ref{lem_bound_v.2} and $\eta^{(t)} = D {\varepsilon}$. Hence, 
\begin{align*}
    \| \epsilon_i^{(t)} \|^2 = \sum_{j=1}^c | \epsilon_{i,j}^{(t)} |^2 \leq c (2+(V+\delta +2) G D^2 \varepsilon)^2\varepsilon^2  . 
\end{align*}
\end{proof}





\begin{lem}\label{lem_main_result_01_new.2}
Suppose that Assumptions \ref{ass_approx_h}, \ref{ass_solve_v} and \ref{ass_bounded_hessian.2} hold. Additionally we assume that $v^{(t)}$ satisfies \peqref{criteria_eps_sol.2}. Consider $\eta^{(t)} = D {\varepsilon}$ for some $D > 0$ and $\varepsilon > 0$; $\alpha_i^{(t)} \leq \frac{\alpha}{L_{\phi}}$, for some $\alpha \in (0, \frac{1}{4})$. For $i = 1,\dots,n$ and $t \geq 0$, we have

\begin{align*}
    \| h(w^{(t+1)};i) - h_i^* \|^2 &\leq  (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ]\\
    & \quad + \varepsilon(4\varepsilon+3)\left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2\right]\\
    & \quad + \frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \tagthis \label{eq_lem_main_result_01_new.2}
\end{align*}



\end{lem}

\begin{proof}
Note that $v^{(t)}$ is obtained from the optimization problem \peqref{opt_prob_L2} for $t \geq 0$. From \peqref{eq_002.1}, we have, for $i = 1,\dots,n$,
\begin{align*}
    h(w^{(t+1)};i) & =   h(w^{(t)} - \eta^{(t)} v^{(t)} ;i) \\
    %
    & = h(w^{(t)};i) - H_i^{(t)} \eta^{(t)} v^{(t)} + \epsilon_i^{(t)} \\
    %
    &= h(w^{(t)};i) - \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) + \epsilon_i^{(t)} \\ & \qquad - [ H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) ]. 
\end{align*}

Hence, we have
\allowdisplaybreaks
\begin{align*}
    &\qquad \| h(w^{(t+1)};i) - h_i^* \|^2\\
    &= \| h(w^{(t)};i) - h_i^* - \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \\&\qquad + \epsilon_i^{(t)}  - [ H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) ] \|^2 \\
    %
    &= \| h(w^{(t)};i) - h_i^* \|^2 +  \| \eta^{(t)}  H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2  + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2  \\ & \quad + \| \epsilon_i^{(t)} \|^2+ \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
    %
    & \quad - 2 \cdot \langle h(w^{(t)};i) - h_i^* , \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \rangle \\
    & \quad- 2 \cdot \langle  h(w^{(t)};i) - h_i^* ,\alpha_i^{(t)}  \nabla_x \phi_i (h(w^{(t)};i)) \rangle \\
    & \quad+ 2 \cdot \langle h(w^{(t)};i) - h_i^* , \epsilon_i^{(t)} \rangle  \\
    & \quad- 2 \cdot\langle h(w^{(t)};i) - h_i^* , H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \rangle \\
    %
    & \quad + 2 \cdot \langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) ,  \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \rangle \\
    & \quad - 2 \cdot\langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) , \epsilon_i^{(t)} \rangle \\
    & \quad + 2 \cdot \langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}), H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \rangle \\
    %
    & \quad- 2 \cdot \langle \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) , \epsilon_i^{(t)} \rangle \\
    & \quad + 2 \cdot \langle \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)), H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \rangle \\
    & \quad - 2 \cdot\langle \epsilon_i^{(t)}, H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \rangle,
\end{align*}
where we expand the square term. Now applying Young's inequalities: $2| \langle u , v \rangle |  \leq \frac{\| u \|^2}{\varepsilon/3} + (\varepsilon/3) \| v \|^2$ for $\varepsilon > 0$ and $2| \langle u , v \rangle | \leq \| u \|^2 + \| v \|^2$ we have:
\begin{align*}
    &\qquad \| h(w^{(t+1)};i) - h_i^* \|^2\\
    %
    &= \| h(w^{(t)};i) - h_i^* \|^2 +  \|\eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2  + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2  \\ & \quad + \| \epsilon_i^{(t)} \|^2+ \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
    %
   & \quad + \frac{\varepsilon}{3} \| h(w^{(t)};i) - h_i^* \|^2 + \frac{3}{\varepsilon} \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \|^2 \\ 
    & \quad - 2 \alpha_i^{(t)} \langle  h(w^{(t)};i) - h_i^* , \nabla_x \phi_i (h(w^{(t)};i)) \rangle\\ 
    & \quad
    + \frac{\varepsilon}{3} \| h(w^{(t)};i) - h_i^* \|^2 +  \frac{3}{\varepsilon} \| \epsilon_i^{(t)} \|^2 \\
    & \quad + \frac{\varepsilon}{3} \| h(w^{(t)};i) - h_i^* \|^2 + \frac{3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2\\
    %
    & \quad + 3 ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 + 3 ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + 3 \| \epsilon_i^{(t)} \|^2 \\
    & \quad + 3 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
    %
    & \overset{\peqref{eq_phi_convex}}{\leq} (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2  + 4 ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2\\
    & \quad +\left( 4+ \frac{3}{\varepsilon} \right)\| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \|^2 + \left( 4+ \frac{3}{\varepsilon} \right) \| \epsilon_i^{(t)} \|^2  \\
    & \quad + \left( 4+ \frac{3}{\varepsilon} \right) \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\ 
    & \quad - 2 \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] 
\end{align*}

Note that from \peqref{eq_phi_convex_smooth} we get that $\| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \leq 2 L_{\phi} [ \phi_i (h(w^{(t)};i)) - \phi_i (h_i^* ) ]$. Applying this and using the fact that $\alpha_i^{(t)} \leq \frac{\alpha}{L_{\phi}}$, for some $\alpha \in (0, \frac{1}{4})$, we are able to derive:
\begin{align*}
    &\qquad \| h(w^{(t+1)};i) - h_i^* \|^2 \\
    %
    & \leq (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ] \\
    & \quad +\frac{4\varepsilon+3}{\varepsilon}\| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \|^2 + \frac{4\varepsilon+3}{\varepsilon}\| \epsilon_i^{(t)} \|^2  \\
    & \quad + \frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\ 
    %
    & \overset{(a)}{\leq} (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ]\\
    & \quad +\frac{4\varepsilon+3}{\varepsilon} D^2\varepsilon^2 H^2 \| v^{(t)} - v_{*\ \text{reg}}^{(t)}  \|^2 + \frac{4\varepsilon+3}{\varepsilon}\| \epsilon_i^{(t)} \|^2  \\
    & \quad + \frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
    %
    & \overset{(b)}{\leq} (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ]\\
    & \quad +\frac{4\varepsilon+3}{\varepsilon} D^2 H^2 \cdot \delta\varepsilon^2 + \frac{4\varepsilon+3}{\varepsilon} \cdot c(2+(V+\delta +2) G D^2 \varepsilon)^2 \varepsilon^2  \\
    & \quad + \frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
    %
    & = (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ]\\
    & \quad +  \varepsilon(4\varepsilon+3)\left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2\right] \\
    & \quad + \frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 
\end{align*}

where
 $(a)$ follows by using matrix vector inequality $\| H v \| \leq \| H \| \|v \| $, where $H \in \mathbb{R}^{c \times d}$ and $v \in \mathbb{R}^d$ and Assumption~\ref{ass_bounded_hessian.2} in \peqref{eq_ass_bounded_hessian.2} and $\eta^{(t)} = D {\varepsilon}$ for some $D > 0$ and $\varepsilon > 0$; $(b)$ follows by the fact that $\| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2 \leq \delta$ in  \peqref{criteria_eps_sol.2} and Lemma \ref{lem_bound_epsilon.2}. 
\end{proof}






\begin{lem}\label{lem_main_result_02_new.2}


Suppose that Assumptions \ref{ass_approx_h}, \ref{ass_solve_v} and \ref{ass_bounded_hessian.2} hold. Additionally we assume that $v^{(t)}$ satisfies \peqref{criteria_eps_sol.2}. Consider $\eta^{(t)} = D {\varepsilon}$ for some $D > 0$ and $\varepsilon > 0$ and the learning rate satisfies:
\begin{align*}
    \alpha_i^{(t)} = ( 1 + \varepsilon ) \alpha_i^{(t-1)} = ( 1 + \varepsilon )^t \alpha_i^{(0)}, \ t = 1,\dots,T  %\tagthis \label{learning_rate_power}
\end{align*}
for $\varepsilon > 0$ with $T = \frac{\beta}{\varepsilon}$ and $\alpha_i^{(0)} = \frac{\alpha}{e^{\beta} L_{\phi}}$ for some constant $\beta > 0$, $\alpha \in (0, \frac{1}{4})$.

We have
\allowdisplaybreaks

\begin{align*}
    & \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ]\\ 
    & \leq  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon\\
    & \quad + \frac{e^{\beta} L_{\phi}(4\varepsilon+3)}{2\alpha( 1 - 4 \alpha)}   \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2 + 2+ V\right] \cdot \varepsilon. \tagthis \label{eq_lem_main_result_02_new.2}
\end{align*}
\end{lem}

\begin{proof}
Rearranging the terms in Lemma~\ref{lem_main_result_01_new.2},
we have
\allowdisplaybreaks
\begin{align*}
     \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) & \leq \frac{1}{2 ( 1 - 4 \alpha)}\left( \frac{(1 + \varepsilon)}{\alpha_i^{(t)}} \| h(w^{(t)};i) - h_i^* \|^2 - \frac{1}{\alpha_i^{(t)}} \| h(w^{(t+1)};i) - h_i^* \|^2 \right) \\
    & \quad + \frac{1}{2( 1 - 4 \alpha)} \cdot \frac{1}{\alpha_i^{(t)}} \cdot \varepsilon(4\varepsilon+3) \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2\right] \\
    & \quad
    + \frac{1}{2( 1 - 4 \alpha)} \cdot \frac{1}{\alpha_i^{(t)}} \cdot\frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2   \\
    %
    & \leq \frac{1}{2 ( 1 - 4 \alpha)}\left( \frac{(1 + \varepsilon)}{\alpha_i^{(t)}}  \| h(w^{(t)};i) - h_i^* \|^2 - \frac{(1 + \varepsilon)}{\alpha_i^{(t+1)}} \| h(w^{(t+1)};i) - h_i^* \|^2 \right) \\
    & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot \varepsilon(4\varepsilon+3) \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2\right] \\
    & \quad
    + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot\frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 .
    \tagthis \label{eq_0001_new.2}
\end{align*}
The last inequality follows because the learning rate satisfies $\alpha_i^{(0)} = \frac{\alpha}{e^{\beta} L_{\phi}} \leq \frac{\alpha}{L_{\phi}}$ and for $t = 1,\dots,T = \frac{\beta}{\varepsilon}$ for some $\beta > 0$
\begin{align*}
    \alpha_i^{(t)} = ( 1 + \varepsilon ) \alpha_i^{(t-1)} = ( 1 + \varepsilon )^t \alpha_i^{(0)} \leq ( 1 + \varepsilon )^T \alpha_i^{(0)} = ( 1 + \varepsilon )^{\beta/\varepsilon} \frac{\alpha}{e^{\beta} L_{\phi}} \leq \frac{\alpha}{L_{\phi}}, 
\end{align*}
since $(1 + x)^{1/x} \leq e$, $x > 0$. Moreover, we have $\frac{1}{\alpha_i^{(t)}} \leq \frac{1}{\alpha_i^{(0)}} = \frac{e^{\beta} L_{\phi}}{\alpha}$, $t = 0,\dots,T-1$. 

Taking the average sum from $t = 0,\dots,T-1$, we have
\begin{align*}
    \frac{1}{T} \sum_{t=0}^{T-1} [\phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] & \leq \frac{1}{2 ( 1 - 4 \alpha) T} \cdot \frac{( 1 + \varepsilon ) }{\alpha_i^{(0)}} \| h(w^{(0)};i) - h_i^* \|^2 \\
    & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot \varepsilon(4\varepsilon+3) \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2\right] \\
    & \quad
    + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot\frac{4\varepsilon+3}{\varepsilon} \frac{1}{T} \sum_{t=0}^{T-1} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
    %
    & = \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \cdot \| h(w^{(0)};i) - h_i^* \|^2 \\
    & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot \varepsilon(4\varepsilon+3) \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2\right] \\
    & \quad
    + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot\frac{4\varepsilon+3}{\varepsilon} \frac{1}{T} \sum_{t=0}^{T-1} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2.
\end{align*}
Taking the average sum from $i = 1,\dots,n$, we have
\begin{align*}
    & \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  \\ 
    & \leq \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \\
    & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot \varepsilon(4\varepsilon+3) \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2\right] \\
    & \quad
    + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot\frac{4\varepsilon+3}{\varepsilon} \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n  \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2\\
    %
    & \overset{\peqref{eq_lem_stronglyconvex_prob}}{\leq}  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \\
    & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot \varepsilon(4\varepsilon+3) \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2\right] \\
    & \quad
    + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot\frac{4\varepsilon+3}{\varepsilon} (2+V) \varepsilon^2. \tagthis \label{eq_0002_new.2}
\end{align*}

Note that
\begin{align*}
     \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  = \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ]. \tagthis \label{eq_average_phi_02.2}
\end{align*}

Therefore, applying \peqref{eq_average_phi_02.2} to \peqref{eq_0002_new.2}, we have
\begin{align*}
    & \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] \\ 
    & \leq  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta}  \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon\\
    & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  (4\varepsilon+3) \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2 + 2+ V\right]\cdot \varepsilon . %\tagthis \label{eq_0002_new}
\end{align*}
\end{proof}



\subsection*{Proof of Theorem~\ref{thm_main_result_GD_solved.2}}

% \begin{thm}\label{thm_main_result_GD_solved.2}
% % Suppose that Assumptions ... hold and Assumption~\ref{ass_diff_optimal_eps} holds with $\delta = P \varepsilon$ for some $P > 0$ and $\varepsilon > 0$. 
% Suppose that Assumptions \ref{ass_approx_h}, \ref{ass_solve_v}, \ref{ass_diff_optimal_eps} and \ref{ass_bounded_hessian.2} hold. Additionally we assume that $v^{(t)}$ satisfies \peqref{criteria_eps_sol.2}. Consider $\eta^{(t)} = D{\varepsilon}$ for some $D > 0$ and $\varepsilon > 0$ and the learning rate satisfies:
% \begin{align*}
%     \alpha_i^{(t)} = ( 1 + \varepsilon ) \alpha_i^{(t-1)} = ( 1 + \varepsilon )^t \alpha_i^{(0)}, \ t = 1,\dots,T  %\tagthis \label{learning_rate_power}
% \end{align*}
% for $\varepsilon > 0$ with $T = \frac{\beta}{\varepsilon}$ and $\alpha_i^{(0)} = \frac{\alpha}{e^{\beta} L_{\phi}}$ for some constant $\beta > 0$, $\alpha \in (0, \frac{1}{4})$.

% We have
% \allowdisplaybreaks

% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] & \leq  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon \\% + P \varepsilon \\
%     & \quad + \frac{e^{\beta} L_{\phi}(4\varepsilon+3)}{2\alpha( 1 - 4 \alpha)}  \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2 + 2+ V\right] \cdot \varepsilon.  \tagthis \label{eq_thm_main_result_GD_solved_new.2}
% \end{align*}


% \end{thm}

\begin{proof}
We have 
\allowdisplaybreaks
\begin{align*}
    \frac{1}{T} \sum_{t=1}^{T} [ F (w^{(t)}) - F_* ] & = \frac{1}{T} \sum_{t=1}^{T} \left( \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] - \left[ F_* - \frac{1}{n} \sum_{i=1}^{n} \phi_i (h_i^* )  \right] \right) \\
    & \overset{\peqref{eq_loss_great_01}}{\leq} \frac{1}{T} \sum_{t=1}^{T} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] \\% + P \varepsilon \\
    % 
    & \overset{\peqref{eq_lem_main_result_02_new.2}%,\peqref{eq_ass_diff_optimal_eps}
    }{\leq}  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon \\% + P \varepsilon \\
    & \quad + \frac{e^{\beta} L_{\phi}(4\varepsilon+3)}{2\alpha( 1 - 4 \alpha)}  \left[\delta D^2H^2 + c (2+(V+\delta +2) G D^2 \varepsilon)^2 + 2+ V\right] \cdot \varepsilon. 
\end{align*}

\end{proof}




% ======= OLD ANALYSIS (START) ===============

% % ==========================================================
% % Proof for Theorem GD_solved
% % ==========================================================

% \section{Technical Proofs for Theorem \ref{thm_main_result_GD_solved}}\label{sec_proofs_GD_solved}
% % \subsection*{Proof of Lemmas}

% \begin{ass}\label{ass_bounded_hessian}
% Let $H_i^{(t)}$ be the Jacobian matrix defined in Lemma~\ref{lem_approx_h}.
% For $i = 1,\dots,n$ and $t \geq 0$, we assume that
% \begin{align*}
%     \| H_i^{(t)} \| \leq \frac{H}{\sqrt{\varepsilon}}, \tagthis \label{eq_ass_bounded_hessian}
% \end{align*}
% for some $H > 0$ and $\varepsilon > 0$. 
% \end{ass}

% Since function $\Psi$ is $\varepsilon^2$-strongly convex, we have, for $\forall v \in \mathbb{R}^d$, 
% \begin{align*}
%     \Psi(v) - \Psi(v_*) \geq \frac{\varepsilon^2}{2} \| v - v_* \|^2, \tagthis \label{eq_strongly_convex_01}
% \end{align*}
% where $v_*$ is the optimal solution of $\Psi$. Hence, by using $\frac{1}{2}\| a \|^2 - \| b \|^2 \leq \| a - b \|^2$, we have
% \begin{align*}
%     \| v \|^2 \leq \frac{4}{\varepsilon^2} [\Psi(v) - \Psi(v_*)] + 2 \| v_* \|^2. \tagthis \label{eq_strongly_convex_02}
% \end{align*}

% Notice that, for strongly convex problem we can find $v^{(t)}$ so that, for $t \geq 0$,
% \begin{align*}
%      \Psi(v^{(t)}) - \Psi(v_{*\ \text{reg}}^{(t)}) \leq \varepsilon^4, \tagthis \label{criteria_eps_sol}
% \end{align*}
% by using Gradient Descent in $\mathcal{O}(n \kappa \log(1/\varepsilon^4))$ number of gradient evaluations \textbf{[CITE THIS, e.g. Nesterov's lecture]}, where $\kappa$ is the condition number. 
% Note that
% \begin{align*}
%     \nabla_v \psi_i (v) = \eta^{(t)} H_i^{(t)}{^\top} [ H_i^{(t)} \eta^{(t)} v - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) ], \ i = 1,\dots,n. \tagthis \label{eq_grad_v}
% \end{align*}
% Note that
% \begin{align*}
%     H_i^{(t)}{^\top} H_i^{(t)} = \left(  \sum_{j=1}^{c} \frac{\partial h(w^{(t)} ; i)_j}{\partial w_{m_r}} \cdot \frac{\partial h(w^{(t)} ; i)_j}{\partial w_{m_c}} \right) \ , \ m_r = 1,\dots,d, \ m_c = 1,\dots,d. \tagthis \label{matrix_H_H}
% \end{align*}
% Consider $\eta^{(t)} = C \sqrt{\varepsilon}$ for some $C > 0$ and $\varepsilon > 0$, we have for $i = 1,\dots,n$ and $t \geq 0$
% \begin{align*}
%     \| \nabla^2_v \psi_i^{(t)} ( v ) \| = (\eta^{(t)})^2 \| H_i^{(t)}{^\top} H_i^{(t)} \| \leq (\eta^{(t)})^2 \| H_i^{(t)} \| \cdot \| H_i^{(t)} \| \overset{\peqref{eq_ass_bounded_hessian}}{\leq} C^2 H^2. 
% \end{align*}

% Hence, $L = C^2 H^2 + \varepsilon^2$ and $\kappa = \frac{L}{\varepsilon^2} = \frac{C^2 H^2 + \varepsilon^2}{\varepsilon^2}$. Hence, the complexity to find $\Psi(v^{(t)}) - \Psi(v_{*\ \text{reg}}^{(t)}) \leq \varepsilon^4$ is $\mathcal{O}(\frac{n (C^2 H^2 + \varepsilon^2)}{\varepsilon^2} \log(1/\varepsilon^4))$. 

% \renewcommand{\thealgorithm}{2}
% \begin{algorithm}[hpt!]
%   \caption{Solve the regularized problem using Gradient Descent}
%   \label{alg_GD_solved}
% \begin{algorithmic}
%   \STATE {\bfseries Initialization:} Choose an initial point $w^{(0)}\in\R^d$, tolerance $\varepsilon > 0$;
%   \FOR{$t=0,1,\cdots,T-1 $}
%   \STATE Use Gradient Descent algorithm to solve the problem \peqref{opt_prob_L2} and find a solution $v^{(t)}$ that satisfies 
%   $$\Psi(v^{(t)}) - \Psi(v_{*\ \text{reg}}^{(t)}) \leq \varepsilon^4$$
%   \STATE Update $w^{(t+1)} = w^{(t)} - \eta^{(t)} v^{(t)}$
%   \ENDFOR
% %   \STATE\textbf{Output:} 
% % Choose $\hat{w}_T \in \{ w^{(0)},\cdots,w^{(T-1)}\}$ uniformly at random.
% \end{algorithmic}
% \end{algorithm} 





% \begin{thm}\label{thm_main_result_GD_solved}
% % Suppose that Assumptions ... hold and Assumption~\ref{ass_diff_optimal_eps} holds with $\delta = P \varepsilon$ for some $P > 0$ and $\varepsilon > 0$. 
% Suppose that Assumptions \ref{ass_approx_h}, \ref{ass_solve_v}, \ref{ass_diff_optimal_eps} and \ref{ass_bounded_hessian} hold. Additionally we assume that $v^{(t)}$ satisfies \peqref{criteria_eps_sol}. Consider $\eta^{(t)} = C \sqrt{\varepsilon}$ for some $C > 0$ and $\varepsilon > 0$ and the learning rate satisfies:
% \begin{align*}
%     \alpha_i^{(t)} = ( 1 + \varepsilon ) \alpha_i^{(t-1)} = ( 1 + \varepsilon )^t \alpha_i^{(0)}, \ t = 1,\dots,T  %\tagthis \label{learning_rate_power}
% \end{align*}
% for $\varepsilon > 0$ with $T = \frac{\beta}{\varepsilon}$ and $\alpha_i^{(0)} = \frac{\alpha}{e^{\beta} L_{\phi}}$ for some constant $\beta > 0$, $\alpha \in (0, \frac{1}{4})$.

% We have
% \allowdisplaybreaks
% % \begin{align*}
% %     \frac{1}{T} \sum_{t=1}^T [ F (w^{(t)}) - F_* ]
% %     & \leq \left( \frac{e^{\beta} L_{\phi} (1 + \varepsilon)}{2 ( 1 - 4 \alpha) \alpha \beta} \frac{1}{n} \sum_{i=1}^n \| h(w^{(0)};i) - h_i^* \|^2 \right) \varepsilon \\
% %     & \quad + \frac{e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \Big ( 8 C^2 H^2 \varepsilon^2 \\
% %     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 \\
% %     & \quad + 6 C^2 H^2 \varepsilon +  12 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon \\
% %     & \quad + 8 (1 + \frac{V}{2}) \varepsilon^2 + 6 (1 + \frac{V}{2}) \varepsilon \Big) \\
% %     & \quad + \frac{4 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha}  \varepsilon^2 + \frac{2 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha)\alpha} \varepsilon^2 \\
% %     & \quad + \frac{3 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha} \varepsilon + \frac{6 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon \\
% %     & \quad + \frac{4 (1 + \frac{V}{2}) e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon^2 + \frac{3 ( 1 + \frac{V}{2} ) e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha) \alpha} \varepsilon + P \varepsilon. \tagthis \label{eq_thm_main_result_01_new}
% % \end{align*}
% % Simpler form
% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] & \leq  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon \\% + P \varepsilon \\
%     & \quad + \frac{e^{\beta} L_{\phi}(4\varepsilon+3) }{8\alpha( 1 - 4 \alpha)} \left[8C^2 H^2 + c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2 + 8+ 4V\right] \cdot \varepsilon. \tagthis \label{eq_thm_main_result_GD_solved_new}
% \end{align*}


% \end{thm}

% \textcolor{blue}{ \bf Proof of Theorem 1 is in Appendix \ref{sec_proofs_GD_solved}}
% \begin{cor}\label{cor_thm_main_result_GD_solved_new}
% Suppose that the conditions in Theorem~\ref{thm_main_result_GD_solved} hold. Then, the total complexity to guarantee
% \begin{align*}
%     \min_{1 \leq t \leq T} [ F (w^{(t)}) - F_* ] \leq \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] \leq \mathcal{O}(\varepsilon)
% \end{align*}
% is $\mathcal{O}\left(\frac{n (C^2 H^2 + \varepsilon^2)}{\varepsilon^3} \log(1/\varepsilon^4) \right)$. 
% \end{cor}

% \begin{proof}
% It is clear that from \peqref{eq_thm_main_result_GD_solved_new}, we have
% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] \leq \mathcal{O}(\varepsilon)
% \end{align*}
% after $T = \frac{\beta}{\varepsilon}$ for some $\beta > 0$. Hence, the total complexity is $\mathcal{O}\left(\frac{n (C^2 H^2 + \varepsilon^2)}{\varepsilon^3} \log(1/\varepsilon^4) \right)$.
% \end{proof}




% \begin{lem}\label{lem_bound_v}
% For $t \geq 0$, suppose that Assumption  \ref{ass_solve_v} holds and $v^{(t)}$ satisfies \peqref{criteria_eps_sol}. Hence, 
% \begin{enumerate}
%     \item $\| v^{(t)} \|^2 \leq 4 \varepsilon^2 + 4 + 2 V$, 
%     \item $ \| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2 \leq 2 \varepsilon^2$. 
% \end{enumerate}
% \end{lem}

% \begin{proof}
% 1) By \peqref{eq_strongly_convex_02}, we have
% \begin{align*}
%     \| v^{(t)} \|^2 \leq \frac{4}{\varepsilon^2} [\Psi(v^{(t)}) - \Psi(v_{*\ \text{reg}}^{(t)})] + 2 \| v_{*\ \text{reg}}^{(t)} \|^2 \overset{\peqref{criteria_eps_sol}}{\leq} 4 \varepsilon^2 + 4 + 2 V,
% \end{align*}
% where the last inequality follows since $\| v_{*\ \text{reg}}^{(t)} \|^2 \leq 2+ V$ for some $V > 0$ in Lemma~\ref{lem_stronglyconvex_prob}. 

% 2) By \peqref{eq_strongly_convex_01}, we have
% \begin{align*}
%      \| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2 \leq \frac{2}{\varepsilon^2} [\Psi(v^{(t)}) - \Psi(v_{*\ \text{reg}}^{(t)})] \leq 2 \varepsilon^2. 
% \end{align*}
% \end{proof}

% \begin{lem}\label{lem_bound_epsilon}
% Suppose that Assumptions~\ref{ass_approx_h} and \ref{ass_solve_v} hold. Consider $\eta^{(t)} = C \sqrt{\varepsilon}$ for some $C > 0$ and $\varepsilon > 0$. For $i = 1,\dots,n$ and $t \geq 0$, we have
% \begin{align*}
%     \| \epsilon_i^{(t)} \|^2 \leq \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2\varepsilon^2. \tagthis \label{eq_lem_bound_epsilon}
% \end{align*}
% \end{lem}

% \begin{proof}
% From \peqref{eq_epsilon}, for $i = 1,\dots,n$, $j = 1,\dots,c$, and $\forall t \geq 0$, by Lemma~\ref{lem_approx_h} we have
% \begin{align*}
%     | \epsilon_{i,j}^{(t)} | & \leq  \frac{1}{2}(\eta^{(t)})^2 \| v^{(t)} \|^2 G + 2\varepsilon \leq \frac{1}{2}(4 \varepsilon^2 + 4 + 2 V) G C^2 \varepsilon + 2\varepsilon \leq \frac{1}{2}\varepsilon (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 ) ,  
% \end{align*}
% where the last inequality follows by the application of Lemma~\ref{lem_bound_v} and $\eta^{(t)} = C \sqrt{\varepsilon}$. Hence, 
% \begin{align*}
%     \| \epsilon_i^{(t)} \|^2 = \sum_{j=1}^c | \epsilon_{i,j}^{(t)} |^2 \leq \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2\varepsilon^2  . 
% \end{align*}
% \end{proof}

% \begin{lem}\label{lem_main_result_01_new}
% Suppose that Assumptions \ref{ass_approx_h}, \ref{ass_solve_v} and \ref{ass_bounded_hessian} hold. Additionally we assume that $v^{(t)}$ satisfies \peqref{criteria_eps_sol}. Consider $\eta^{(t)} = C \sqrt{\varepsilon}$ for some $C > 0$ and $\varepsilon > 0$; $\alpha_i^{(t)} \leq \frac{\alpha}{L_{\phi}}$, for some $\alpha \in (0, \frac{1}{4})$. For $i = 1,\dots,n$ and $t \geq 0$, we have
% % \begin{align*}
% %     \| h(w^{(t+1)};i) - h_i^* \|^2 & \leq (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 + 8 C^2 H^2 \varepsilon^2 \\
% %     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 + 4 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
% %     & \quad + 6 C^2 H^2 \varepsilon +  12 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon \\
% %     & \quad + \frac{3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\ 
% %     & \quad - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ]. \tagthis \label{eq_lem_main_result_01_new}
% % \end{align*}
% % Simpler expression:
% \begin{align*}
%     \| h(w^{(t+1)};i) - h_i^* \|^2 &\leq  (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ]\\
%     & \quad + \frac{ \varepsilon(4\varepsilon+3)}{4} \left[8C^2 H^2 + c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2\right] \\
%     & \quad + \frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \tagthis \label{eq_lem_main_result_01_new}
% \end{align*}



% \end{lem}

% \begin{proof}
% Note that $v^{(t)}$ is obtained from the optimization problem \peqref{opt_prob_L2} for $t \geq 0$. From \peqref{eq_002.1}, we have, for $i = 1,\dots,n$,
% \begin{align*}
%     h(w^{(t+1)};i) & =   h(w^{(t)} - \eta^{(t)} v^{(t)} ;i) \\
%     %
%     & = h(w^{(t)};i) - H_i^{(t)} \eta^{(t)} v^{(t)} + \epsilon_i^{(t)} \\
%     %
%     &= h(w^{(t)};i) - \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) + \epsilon_i^{(t)} \\ & \qquad - [ H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) ]. 
% \end{align*}

% Hence, we have
% \allowdisplaybreaks
% \begin{align*}
%     &\qquad \| h(w^{(t+1)};i) - h_i^* \|^2\\
%     &= \| h(w^{(t)};i) - h_i^* - \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \\&\qquad + \epsilon_i^{(t)}  - [ H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) ] \|^2 \\
%     %
%     &= \| h(w^{(t)};i) - h_i^* \|^2 +  \| \eta^{(t)}  H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2  + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2  \\ & \quad + \| \epsilon_i^{(t)} \|^2+ \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     %
%     & \quad - 2 \cdot \langle h(w^{(t)};i) - h_i^* , \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \rangle \\
%     & \quad- 2 \cdot \langle  h(w^{(t)};i) - h_i^* ,\alpha_i^{(t)}  \nabla_x \phi_i (h(w^{(t)};i)) \rangle \\
%     & \quad+ 2 \cdot \langle h(w^{(t)};i) - h_i^* , \epsilon_i^{(t)} \rangle  \\
%     & \quad- 2 \cdot\langle h(w^{(t)};i) - h_i^* , H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \rangle \\
%     %
%     & \quad + 2 \cdot \langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) ,  \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \rangle \\
%     & \quad - 2 \cdot\langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) , \epsilon_i^{(t)} \rangle \\
%     & \quad + 2 \cdot \langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}), H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \rangle \\
%     %
%     & \quad- 2 \cdot \langle \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) , \epsilon_i^{(t)} \rangle \\
%     & \quad + 2 \cdot \langle \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)), H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \rangle \\
%     & \quad - 2 \cdot\langle \epsilon_i^{(t)}, H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \rangle,
%     % %
%     % & \overset{(a)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     % & \quad + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + \| \epsilon_i^{(t)} \|^2 \\
%     % & \quad + \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     % & \quad + 2 \| h(w^{(t)};i) - h_i^* \| \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \| \\ & \quad - 2 \alpha_i^{(t)} \langle  h(w^{(t)};i) - h_i^* , \nabla_x \phi_i (h(w^{(t)};i)) \rangle + 2 \| h(w^{(t)};i) - h_i^* \| \| \epsilon_i^{(t)} \| \\
%     % & \quad + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     % & \quad + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 + \| \epsilon_i^{(t)} \|^2 \\
%     % & \quad + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + \| \epsilon_i^{(t)} \|^2 \\
%     % & \quad + 2 \| h(w^{(t)};i) - h_i^* \| \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \| \\
%     % & \quad + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 + \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
%     % & \quad + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2  \\
%     % & \quad + \| \epsilon_i^{(t)} \|^2 + \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
% \end{align*}
% where we expand the square term. Now applying Young's inequalities: $2| \langle u , v \rangle |  \leq \frac{\| u \|^2}{\varepsilon/3} + (\varepsilon/3) \| v \|^2$ for $\varepsilon > 0$ and $2| \langle u , v \rangle | \leq \| u \|^2 + \| v \|^2$ we have:
% \begin{align*}
%     &\qquad \| h(w^{(t+1)};i) - h_i^* \|^2\\
%     %
%     &= \| h(w^{(t)};i) - h_i^* \|^2 +  \|\eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2  + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2  \\ & \quad + \| \epsilon_i^{(t)} \|^2+ \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     %
%   & \quad + \frac{\varepsilon}{3} \| h(w^{(t)};i) - h_i^* \|^2 + \frac{3}{\varepsilon} \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \|^2 \\ 
%     & \quad - 2 \alpha_i^{(t)} \langle  h(w^{(t)};i) - h_i^* , \nabla_x \phi_i (h(w^{(t)};i)) \rangle\\ 
%     & \quad
%     + \frac{\varepsilon}{3} \| h(w^{(t)};i) - h_i^* \|^2 +  \frac{3}{\varepsilon} \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + \frac{\varepsilon}{3} \| h(w^{(t)};i) - h_i^* \|^2 + \frac{3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2\\
%     %
%     & \quad + 3 ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 + 3 ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + 3 \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + 3 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     %
%     & \overset{\peqref{eq_phi_convex}}{\leq} (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2  + 4 ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2\\
%     & \quad +\left( 4+ \frac{3}{\varepsilon} \right)\| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \|^2 + \left( 4+ \frac{3}{\varepsilon} \right) \| \epsilon_i^{(t)} \|^2  \\
%     & \quad + \left( 4+ \frac{3}{\varepsilon} \right) \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\ 
%     & \quad - 2 \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] 
% \end{align*}

% Note that from \peqref{eq_phi_convex_smooth} we get that $\| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \leq 2 L_{\phi} [ \phi_i (h(w^{(t)};i)) - \phi_i (h_i^* ) ]$. Applying this and using the fact that $\alpha_i^{(t)} \leq \frac{\alpha}{L_{\phi}}$, for some $\alpha \in (0, \frac{1}{4})$, we are able to derive:
% \begin{align*}
%     &\qquad \| h(w^{(t+1)};i) - h_i^* \|^2 \\
%     %
%     & \leq (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ] \\
%     & \quad +\frac{4\varepsilon+3}{\varepsilon}\| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \|^2 + \frac{4\varepsilon+3}{\varepsilon}\| \epsilon_i^{(t)} \|^2  \\
%     & \quad + \frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\ 
%     %
%     & \overset{(a)}{\leq} (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ]\\
%     & \quad +\frac{4\varepsilon+3}{\varepsilon} C^2 H^2 \| v^{(t)} - v_{*\ \text{reg}}^{(t)}  \|^2 + \frac{4\varepsilon+3}{\varepsilon}\| \epsilon_i^{(t)} \|^2  \\
%     & \quad + \frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     %
%     & \overset{(b)}{\leq} (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ]\\
%     & \quad +\frac{4\varepsilon+3}{\varepsilon} C^2 H^2 \cdot 2\varepsilon^2 + \frac{4\varepsilon+3}{\varepsilon} \cdot \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2 \varepsilon^2  \\
%     & \quad + \frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     %
%     & = (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ]\\
%     & \quad +  \frac{\varepsilon(4\varepsilon+3)}{4}\left[8C^2 H^2 + c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2\right] \\
%     & \quad + \frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 
% \end{align*}
% % Old from Lam
% % \begin{align*}
% %     &\qquad \| h(w^{(t+1)};i) - h_i^* \|^2\\
% %     %
% %     & \leq (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 + 4 ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
% %     & \quad + 4 \| \epsilon_i^{(t)} \|^2 + 4 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
% %     & \quad + \frac{3}{\varepsilon} ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \|^2 +  \frac{3}{\varepsilon} \| \epsilon_i^{(t)} \|^2 + \frac{3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\ 
% %     & \quad - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ] \\
% %     %
% %     & \overset{(a)}{\leq} (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 + 4 C^2 H^2 \| v^{(t)} - v_{*\ \text{reg}}^{(t)}  \|^2 \\
% %     & \quad + 4 \| \epsilon_i^{(t)} \|^2 + 4 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
% %     & \quad + \frac{3}{\varepsilon} C^2 H^2 \| v^{(t)} - v_{*\ \text{reg}}^{(t)} \|^2 +  \frac{3}{\varepsilon} \| \epsilon_i^{(t)} \|^2 + \frac{3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\ 
% %     & \quad - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ] \\
% %     %
% %     & \overset{(b)}{\leq} (1 + \varepsilon) \| h(w^{(t)};i) - h_i^* \|^2 + 8 C^2 H^2 \varepsilon^2 \\
% %     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 + 4 \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
% %     & \quad + 6 C^2 H^2 \varepsilon +  12 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon  + \frac{3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\ 
% %     & \quad - 2 ( 1 - 4 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ],
% % \end{align*}
% where
%  $(a)$ follows by using matrix vector inequality $\| H v \| \leq \| H \| \|v \| $, where $H \in \mathbb{R}^{c \times d}$ and $v \in \mathbb{R}^d$ and Assumption~\ref{ass_bounded_hessian} in \peqref{eq_ass_bounded_hessian} and $\eta^{(t)} = C \sqrt{\varepsilon}$ for some $C > 0$ and $\varepsilon > 0$; $(b)$ follows by Lemmas~\ref{lem_bound_v} and \ref{lem_bound_epsilon}. 
% \end{proof}



% \begin{lem}\label{lem_main_result_02_new}


% Suppose that Assumptions \ref{ass_approx_h}, \ref{ass_solve_v} and \ref{ass_bounded_hessian} hold. Additionally we assume that $v^{(t)}$ satisfies \peqref{criteria_eps_sol}. Consider $\eta^{(t)} = C \sqrt{\varepsilon}$ for some $C > 0$ and $\varepsilon > 0$ and the learning rate satisfies:
% \begin{align*}
%     \alpha_i^{(t)} = ( 1 + \varepsilon ) \alpha_i^{(t-1)} = ( 1 + \varepsilon )^t \alpha_i^{(0)}, \ t = 1,\dots,T  %\tagthis \label{learning_rate_power}
% \end{align*}
% for $\varepsilon > 0$ with $T = \frac{\beta}{\varepsilon}$ and $\alpha_i^{(0)} = \frac{\alpha}{e^{\beta} L_{\phi}}$ for some constant $\beta > 0$, $\alpha \in (0, \frac{1}{4})$.

% We have
% \allowdisplaybreaks
% % \begin{align*}
% %     \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ]
% %     & \leq \left( \frac{e^{\beta} L_{\phi} (1 + \varepsilon)}{2 ( 1 - 4 \alpha) \alpha \beta} \frac{1}{n} \sum_{i=1}^n \| h(w^{(0)};i) - h_i^* \|^2 \right) \varepsilon \\
% %     & \quad + \frac{e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \Big ( 8 C^2 H^2 \varepsilon^2 \\
% %     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 \\
% %     & \quad + 6 C^2 H^2 \varepsilon +  12 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon \\
% %     & \quad + 8 (1 + \frac{V}{2}) \varepsilon^2 + 6 (1 + \frac{V}{2}) \varepsilon \Big) \\
% %     & \quad + \frac{4 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha}  \varepsilon^2 + \frac{2 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha)\alpha} \varepsilon^2 \\
% %     & \quad + \frac{3 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha} \varepsilon + \frac{6 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon \\
% %     & \quad + \frac{4 (1 + \frac{V}{2}) e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon^2 + \frac{3 ( 1 + \frac{V}{2} ) e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha) \alpha} \varepsilon. \tagthis \label{eq_lem_main_result_02_new}
% % \end{align*}
% % Simpler form, and more correct
% \begin{align*}
%     & \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ]\\ 
%     & \leq  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon\\
%     & \quad + \frac{e^{\beta} L_{\phi}(4\varepsilon+3)}{2\alpha( 1 - 4 \alpha)}   \left[2C^2 H^2 +   \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2 + 2+ V\right] \cdot \varepsilon. \tagthis \label{eq_lem_main_result_02_new}
% \end{align*}
% \end{lem}

% \begin{proof}
% Rearranging the terms in Lemma~\ref{lem_main_result_01_new},
% we have
% \allowdisplaybreaks
% % \begin{align*}
% %      \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) & \leq \frac{1}{2 ( 1 - 4 \alpha)}\left( \frac{(1 + \varepsilon)}{\alpha_i^{(t)}} \| h(w^{(t)};i) - h_i^* \|^2 - \frac{1}{\alpha_i^{(t)}} \| h(w^{(t+1)};i) - h_i^* \|^2 \right) \\
% %     & \quad + \frac{1}{\alpha_i^{(t)}} \cdot \frac{4 C^2 H^2}{( 1 - 4 \alpha)}  \varepsilon^2 + \frac{1}{\alpha_i^{(t)}} \cdot \frac{2 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4}{ ( 1 - 4 \alpha)} \varepsilon^2 \\
% %     & \quad + \frac{1}{\alpha_i^{(t)}} \cdot \frac{3 C^2 H^2}{( 1 - 4 \alpha)} \varepsilon +  \frac{1}{\alpha_i^{(t)}} \cdot \frac{6 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4}{( 1 - 4 \alpha)} \varepsilon \\
% %     & \quad + \frac{2}{( 1 - 4 \alpha)} \cdot \frac{1}{\alpha_i^{(t)}} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
% %     & \quad + \frac{3}{2 ( 1 - 4 \alpha) \varepsilon} \cdot \frac{1}{\alpha_i^{(t)}} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
% %     %
% %     & \leq \frac{1}{2 ( 1 - 4 \alpha)}\left( \frac{1}{\alpha_i^{(t-1)}} \| h(w^{(t)};i) - h_i^* \|^2 - \frac{1}{\alpha_i^{(t)}} \| h(w^{(t+1)};i) - h_i^* \|^2 \right) \\
% %     & \quad + \frac{4 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha}  \varepsilon^2 + \frac{2 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha)\alpha} \varepsilon^2 \\
% %     & \quad + \frac{3 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha} \varepsilon + \frac{6 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon \\
% %     & \quad + \frac{2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
% %     & \quad + \frac{3 e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \varepsilon}  \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2.
% %     \tagthis \label{eq_0001_new}
% % \end{align*}
% \begin{align*}
%      \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) & \leq \frac{1}{2 ( 1 - 4 \alpha)}\left( \frac{(1 + \varepsilon)}{\alpha_i^{(t)}} \| h(w^{(t)};i) - h_i^* \|^2 - \frac{1}{\alpha_i^{(t)}} \| h(w^{(t+1)};i) - h_i^* \|^2 \right) \\
%     & \quad + \frac{1}{2( 1 - 4 \alpha)} \cdot \frac{1}{\alpha_i^{(t)}} \cdot \varepsilon(4\varepsilon+3) \left[2C^2 H^2 +   \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2\right] \\
%     & \quad
%     + \frac{1}{2( 1 - 4 \alpha)} \cdot \frac{1}{\alpha_i^{(t)}} \cdot\frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2   \\
%     %
%     & \leq \frac{1}{2 ( 1 - 4 \alpha)}\left( \frac{(1 + \varepsilon)}{\alpha_i^{(t)}}  \| h(w^{(t)};i) - h_i^* \|^2 - \frac{(1 + \varepsilon)}{\alpha_i^{(t+1)}} \| h(w^{(t+1)};i) - h_i^* \|^2 \right) \\
%     & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot \varepsilon(4\varepsilon+3) \left[2C^2 H^2 +   \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2\right] \\
%     & \quad
%     + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot\frac{4\varepsilon+3}{\varepsilon} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 .
%     \tagthis \label{eq_0001_new}
% \end{align*}
% The last inequality follows because the learning rate satisfies $\alpha_i^{(0)} = \frac{\alpha}{e^{\beta} L_{\phi}} \leq \frac{\alpha}{L_{\phi}}$ and for $t = 1,\dots,T = \frac{\beta}{\varepsilon}$ for some $\beta > 0$
% \begin{align*}
%     \alpha_i^{(t)} = ( 1 + \varepsilon ) \alpha_i^{(t-1)} = ( 1 + \varepsilon )^t \alpha_i^{(0)} \leq ( 1 + \varepsilon )^T \alpha_i^{(0)} = ( 1 + \varepsilon )^{\beta/\varepsilon} \frac{\alpha}{e^{\beta} L_{\phi}} \leq \frac{\alpha}{L_{\phi}}, 
% \end{align*}
% since $(1 + x)^{1/x} \leq e$, $x > 0$. Moreover, we have $\frac{1}{\alpha_i^{(t)}} \leq \frac{1}{\alpha_i^{(0)}} = \frac{e^{\beta} L_{\phi}}{\alpha}$, $t = 0,\dots,T-1$. 

% Taking the average sum from $t = 0,\dots,T-1$, we have
% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} [\phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] & \leq \frac{1}{2 ( 1 - 4 \alpha) T} \cdot \frac{( 1 + \varepsilon ) }{\alpha_i^{(0)}} \| h(w^{(0)};i) - h_i^* \|^2 \\
%     & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot \varepsilon(4\varepsilon+3) \left[2C^2 H^2 +   \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2\right] \\
%     & \quad
%     + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot\frac{4\varepsilon+3}{\varepsilon} \frac{1}{T} \sum_{t=0}^{T-1} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     %
%     & = \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \cdot \| h(w^{(0)};i) - h_i^* \|^2 \\
%     & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot \varepsilon(4\varepsilon+3) \left[2C^2 H^2 +   \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2\right] \\
%     & \quad
%     + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot\frac{4\varepsilon+3}{\varepsilon} \frac{1}{T} \sum_{t=0}^{T-1} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2.
% \end{align*}
% Taking the average sum from $i = 1,\dots,n$, we have
% \begin{align*}
%     & \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  \\ 
%     & \leq \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \\
%     & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot \varepsilon(4\varepsilon+3) \left[2C^2 H^2 +   \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2\right] \\
%     & \quad
%     + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot\frac{4\varepsilon+3}{\varepsilon} \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n  \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2\\
%     %
%     & \overset{\peqref{eq_lem_stronglyconvex_prob}}{\leq}  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \\
%     & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot \varepsilon(4\varepsilon+3) \left[2C^2 H^2 +   \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2\right] \\
%     & \quad
%     + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  \cdot\frac{4\varepsilon+3}{\varepsilon} (2+V) \varepsilon^2. \tagthis \label{eq_0002_new}
% \end{align*}
% % Taking the average sum from $t = 1,\dots,T$, we have
% % \begin{align*}
% %     \frac{1}{T} \sum_{t=1}^{T} [\phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] & \leq \frac{1}{2 ( 1 - 4 \alpha) T} \cdot \frac{1}{\alpha_i^{(0)}} \| h(w^{(1)};i) - h_i^* \|^2 \\
% %     & \quad + \frac{4 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha}  \varepsilon^2 + \frac{2 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha)\alpha} \varepsilon^2 \\
% %     & \quad + \frac{3 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha} \varepsilon + \frac{6 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon \\
% %     & \quad + \frac{2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \frac{1}{T} \sum_{t=1}^{T} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
% %     & \quad + \frac{3 e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \varepsilon} \frac{1}{T} \sum_{t=1}^{T}  \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
% %     %
% %     & = \frac{e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \cdot \| h(w^{(1)};i) - h_i^* \|^2 \\
% %     & \quad + \frac{4 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha}  \varepsilon^2 + \frac{2 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha)\alpha} \varepsilon^2 \\
% %     & \quad + \frac{3 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha} \varepsilon + \frac{6 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon \\
% %     & \quad + \frac{2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \frac{1}{T} \sum_{t=1}^{T} \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
% %     & \quad + \frac{3 e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \varepsilon} \frac{1}{T} \sum_{t=1}^{T}  \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2.
% % \end{align*}
% % Taking the average sum from $i = 1,\dots,n$, we have
% % \begin{align*}
% %     & \frac{1}{T} \sum_{t=1}^{T} \frac{1}{n} \sum_{i=1}^n [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  \\ 
% %     & \leq \frac{e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \cdot \frac{1}{n} \sum_{i=1}^n \| h(w^{(1)};i) - h_i^* \|^2 \\
% %     & \quad + \frac{4 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha}  \varepsilon^2 + \frac{2 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha)\alpha} \varepsilon^2 \\
% %     & \quad + \frac{3 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha} \varepsilon + \frac{6 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon \\
% %     & \quad + \frac{2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \frac{1}{T} \sum_{t=1}^{T} \frac{1}{n} \sum_{i=1}^n \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
% %     & \quad + \frac{3 e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \varepsilon} \frac{1}{T} \sum_{t=1}^{T}  \frac{1}{n} \sum_{i=1}^n \| H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))  \|^2 \\
% %     %
% %     & \overset{\peqref{eq_lem_stronglyconvex_prob}}{\leq} \frac{e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \cdot \frac{1}{n} \sum_{i=1}^n \| h(w^{(1)};i) - h_i^* \|^2 \\
% %     & \quad + \frac{4 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha}  \varepsilon^2 + \frac{2 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha)\alpha} \varepsilon^2 \\
% %     & \quad + \frac{3 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha} \varepsilon + \frac{6 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon \\
% %     & \quad + \frac{4 (1 + \frac{V}{2}) e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon^2 + \frac{3 ( 1 + \frac{V}{2} ) e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha) \alpha} \varepsilon. \tagthis \label{eq_0002_new}
% % \end{align*}

% % From Lemma~\ref{lem_main_result_01_new}, with $t = 0$, we have
% % \begin{align*}
% %     \| h(w^{(1)};i) - h_i^* \|^2 & \leq (1 + \varepsilon) \| h(w^{(0)};i) - h_i^* \|^2 + 8 C^2 H^2 \varepsilon^2 \\
% %     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 + 4 \| H_i^{(0)} \eta^{(0)} v_*^{(0)} - \alpha_i^{(0)} \nabla_x \phi_i (h(w^{(0)};i)) \|^2 \\
% %     & \quad + 6 C^2 H^2 \varepsilon +  12 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon \\
% %     & \quad + \frac{3}{\varepsilon} \| H_i^{(0)} \eta^{(0)} v_*^{(0)} - \alpha_i^{(0)} \nabla_x \phi_i (h(w^{(0)};i))  \|^2. 
% % \end{align*}
% % Hence, taking the average sum from $i = 1,\dots,n$, we have
% % \begin{align*}
% %     \frac{1}{n} \sum_{i=1}^n \| h(w^{(1)};i) - h_i^* \|^2 & \leq (1 + \varepsilon) \frac{1}{n} \sum_{i=1}^n \| h(w^{(0)};i) - h_i^* \|^2 + 8 C^2 H^2 \varepsilon^2 \\
% %     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 \\
% %     & \quad + 6 C^2 H^2 \varepsilon +  12 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon \\
% %     & \quad + \frac{4}{n} \sum_{i=1}^n \| H_i^{(0)} \eta^{(0)} v_*^{(0)} - \alpha_i^{(0)} \nabla_x \phi_i (h(w^{(0)};i)) \|^2  \\
% %     & \quad + \frac{3}{\varepsilon} \frac{1}{n} \sum_{i=1}^n \| H_i^{(0)} \eta^{(0)} v_*^{(0)} - \alpha_i^{(0)} \nabla_x \phi_i (h(w^{(0)};i))  \|^2 \\
% %     %
% %     & \overset{\peqref{eq_lem_stronglyconvex_prob}}{\leq} (1 + \varepsilon) \frac{1}{n} \sum_{i=1}^n \| h(w^{(0)};i) - h_i^* \|^2 + 8 C^2 H^2 \varepsilon^2 \\
% %     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 \\
% %     & \quad + 6 C^2 H^2 \varepsilon +  12 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon \\
% %     & \quad + 8 (1 + \frac{V}{2}) \varepsilon^2 + 6 (1 + \frac{V}{2}) \varepsilon. \tagthis \label{eq_0003_new}
% % \end{align*}

% Note that
% \begin{align*}
%      \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  = \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ]. \tagthis \label{eq_average_phi_02}
% \end{align*}

% Therefore, applying \peqref{eq_average_phi_02} to \peqref{eq_0002_new}, we have
% \begin{align*}
%     & \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] \\ 
%     & \leq  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta}  \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon\\
%     & \quad + \frac{e^{\beta} L_{\phi}}{2\alpha( 1 - 4 \alpha)}  (4\varepsilon+3) \left[2C^2 H^2 +   \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2 + 2+ V\right]\cdot \varepsilon . %\tagthis \label{eq_0002_new}
% \end{align*}
% % \begin{align*}
% %     \frac{1}{T} \sum_{t=1}^{T} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] &=  \frac{1}{T} \sum_{t=1}^{T} \frac{1}{n} \sum_{i=1}^n [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] \\
% %     %
% %     & \leq \left( \frac{e^{\beta} L_{\phi} (1 + \varepsilon)}{2 ( 1 - 4 \alpha) \alpha \beta} \frac{1}{n} \sum_{i=1}^n \| h(w^{(0)};i) - h_i^* \|^2 \right) \varepsilon \\
% %     & \quad + \frac{e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \Big ( 8 C^2 H^2 \varepsilon^2 \\
% %     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 \\
% %     & \quad + 6 C^2 H^2 \varepsilon +  12 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon \\ 
% %     & \quad + 8 (1 + \frac{V}{2}) \varepsilon^2 + 6 (1 + \frac{V}{2}) \varepsilon \Big) \\
% %     & \quad + \frac{4 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha}  \varepsilon^2 + \frac{2 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha)\alpha} \varepsilon^2 \\
% %     & \quad + \frac{3 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha} \varepsilon + \frac{6 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon \\
% %     & \quad + \frac{4 (1 + \frac{V}{2}) e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon^2 + \frac{3 ( 1 + \frac{V}{2} ) e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha) \alpha} \varepsilon. 
% % \end{align*}
% \end{proof}



% \subsection*{Proof of Theorem~\ref{thm_main_result_GD_solved}}

% % \begin{thm}\label{thm_main_result_01}
% % % Suppose that Assumptions ... hold and Assumption~\ref{ass_diff_optimal_eps} holds with $\delta = P \varepsilon$ for some $P > 0$ and $\varepsilon > 0$. 
% % Suppose that Assumptions \ref{approx_h}, \ref{ass_solve_v} and \ref{ass_bounded_hessian} hold. Additionally we assume that $v^{(t)}$ satisfies \peqref{criteria_eps_sol} and Assumption~\ref{ass_diff_optimal_eps} holds with $\delta = P \varepsilon$ for some $P > 0$ and $\varepsilon > 0$. Consider $\eta^{(t)} = C \sqrt{\varepsilon}$ for some $C > 0$ and $\varepsilon > 0$ and the learning rate satisfies:
% % \begin{align*}
% %     \alpha_i^{(t)} = ( 1 + \varepsilon ) \alpha_i^{(t-1)} = ( 1 + \varepsilon )^t \alpha_i^{(0)}, \ t = 1,\dots,T  %\tagthis \label{learning_rate_power}
% % \end{align*}
% % for $\varepsilon > 0$ with $T = \frac{\beta}{\varepsilon}$ and $\alpha_i^{(0)} = \frac{\alpha}{e^{\beta} L_{\phi}}$ for some constant $\beta > 0$, $\alpha \in (0, \frac{1}{4})$.

% % We have
% % \allowdisplaybreaks
% % \begin{align*}
% %     \frac{1}{T} \sum_{t=1}^{T} [ F (w^{(t)}) - F_* ]
% %     & \leq \left( \frac{e^{\beta} L_{\phi} (1 + \varepsilon)}{2 ( 1 - 4 \alpha) \alpha \beta} \frac{1}{n} \sum_{i=1}^n \| h(w^{(0)};i) - h_i^* \|^2 \right) \varepsilon \\
% %     & \quad + \frac{e^{\beta} L_{\phi}}{2 ( 1 - 4 \alpha) \alpha \beta} \varepsilon \Big ( 8 C^2 H^2 \varepsilon^2 \\
% %     & \quad + 4 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon^2 \\
% %     & \quad + 6 C^2 H^2 \varepsilon +  12 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 \varepsilon \\
% %     & \quad + 8 (1 + \frac{V}{2}) \varepsilon^2 + 6 (1 + \frac{V}{2}) \varepsilon \Big) \\
% %     & \quad + \frac{4 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha}  \varepsilon^2 + \frac{2 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha)\alpha} \varepsilon^2 \\
% %     & \quad + \frac{3 C^2 H^2 e^{\beta} L_{\phi}}{( 1 - 4 \alpha)\alpha} \varepsilon + \frac{6 c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon \\
% %     & \quad + \frac{4 (1 + \frac{V}{2}) e^{\beta} L_{\phi}}{( 1 - 4 \alpha) \alpha} \varepsilon^2 + \frac{3 ( 1 + \frac{V}{2} ) e^{\beta} L_{\phi}}{ ( 1 - 4 \alpha) \alpha} \varepsilon + P \varepsilon. \tagthis \label{eq_thm_main_result_01_new}
% % \end{align*}
% % Simpler form
% % \begin{align*}
% %     \frac{1}{T} \sum_{t=1}^{T} [ F (w^{(t)}) - F_* ] & \leq  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon \\% + P \varepsilon \\
% %     & \quad + \frac{e^{\beta} L_{\phi}(4\varepsilon+3) }{2\alpha( 1 - 4 \alpha)} \left[2C^2 H^2 + c (4 \varepsilon^2 + 4 + 2 V)^2 G^2 C^4 + 2+ V\right] \cdot \varepsilon. \tagthis \label{eq_thm_main_result_01_new}
% % \end{align*}


% % \end{thm}

% \begin{proof}
% We have
% \allowdisplaybreaks
% \begin{align*}
%     \frac{1}{T} \sum_{t=1}^{T} [ F (w^{(t)}) - F_* ] & = \frac{1}{T} \sum_{t=1}^{T} \left( \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] - \left[ F_* - \frac{1}{n} \sum_{i=1}^{n} \phi_i (h_i^* )  \right] \right) \\
%     & \leq \frac{1}{T} \sum_{t=1}^{T} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] \\% + P \varepsilon \\
%     % 
%     & \overset{\peqref{eq_lem_main_result_02_new},\peqref{eq_ass_diff_optimal_eps}}{\leq}  \frac{e^{\beta} L_{\phi}( 1 + \varepsilon )}{2 ( 1 - 4 \alpha) \alpha \beta} \cdot  \frac{1}{n} \sum_{i=1}^n  \| h(w^{(0)};i) - h_i^* \|^2 \cdot \varepsilon \\% + P \varepsilon \\
%     & \quad + \frac{e^{\beta} L_{\phi}(4\varepsilon+3)}{2\alpha( 1 - 4 \alpha)}  \left[2C^2 H^2 +   \frac{1}{4}c (4+(4 \varepsilon^2 + 4 + 2 V) G C^2 )^2 + 2+ V\right] \cdot \varepsilon. 
% \end{align*}

% \end{proof}

% \begin{cor}\label{cor_thm_main_result_01_new}
% Suppose that the conditions in Theorem~\ref{thm_main_result_01} hold. Then, the total complexity to guarantee
% \begin{align*}
%     \min_{1 \leq t \leq T} [ F (w^{(t)}) - F_* ] \leq \frac{1}{T} \sum_{t=1}^{T} [ F (w^{(t)}) - F_* ] \leq \mathcal{O}(\varepsilon)
% \end{align*}
% is $\mathcal{O}\left(\frac{n (C^2 H^2 + \varepsilon^2)}{\varepsilon^3} \log(1/\varepsilon^4) \right)$. 
% \end{cor}

% \begin{proof}
% It is clear that from \peqref{eq_thm_main_result_01_new}, we have
% \begin{align*}
%     \frac{1}{T} \sum_{t=1}^{T} [ F (w^{(t)}) - F_* ] \leq \mathcal{O}(\varepsilon)
% \end{align*}
% after $T = \frac{\beta}{\varepsilon}$ for some $\beta > 0$. Hence, the total complexity is $\mathcal{O}\left(\frac{n (C^2 H^2 + \varepsilon^2)}{\varepsilon^3} \log(1/\varepsilon^4) \right)$.
% \end{proof}




% Note that $H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} = \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i))$ and $v^{(t)}$ is obtained from the optimization problem \peqref{opt_prob_01}, $t \geq 0$. From \peqref{eq_002.1}, we have, for $i = 1,\dots,n$,
% \begin{align*}
%     h(w^{(t+1)};i) & = x_i^{(t+1)} = x_i^{(t)} =  h(w^{(t)} - \eta^{(t)} v^{(t)} ;i) \\
%     %
%     & = h(w^{(t)};i) - H_i^{(t)} \eta^{(t)} v^{(t)} + \epsilon_i^{(t)} \\
%     %
%     &= h(w^{(t)};i) - \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) + \epsilon_i^{(t)}. 
% \end{align*}

% \lam{Need to change to: 
% \begin{align*}
%     h(w^{(t+1)};i) & = x_i^{(t+1)} = x_i^{(t)} =  h(w^{(t)} - \eta^{(t)} v^{(t)} ;i) \\
%     %
%     & = h(w^{(t)};i) - H_i^{(t)} \eta^{(t)} v^{(t)} + \epsilon_i^{(t)} \\
%     %
%     &= h(w^{(t)};i) - \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) - [ H_i^{(t)} \eta^{(t)} v_{*\ \text{reg}}^{(t)} - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) ] \\ & \qquad - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) + \epsilon_i^{(t)}. 
% \end{align*}

% }

% Hence, we have
% \allowdisplaybreaks
% \begin{align*}
%     \| h(w^{(t+1)};i) - h_i^* \|^2 &= \| h(w^{(t)};i) - h_i^* - \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) - \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) + \epsilon_i^{(t)} \|^2 \\
%     &= \| h(w^{(t)};i) - h_i^* \|^2 + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     & \quad + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + \| \epsilon_i^{(t)} \|^2 \\
%     & \quad - 2 \langle h(w^{(t)};i) - h_i^* , \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \rangle \\ & \quad - 2 \alpha_i^{(t)} \langle  h(w^{(t)};i) - h_i^* , \nabla_x \phi_i (h(w^{(t)};i)) \rangle + 2 \langle h(w^{(t)};i) - h_i^* , \epsilon_i^{(t)} \rangle \\
%     & \quad + 2  \langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) ,  \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) \rangle \\
%     & \quad - 2 \langle \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) , \epsilon_i^{(t)} \rangle - 2  \langle \alpha_i^{(t)} \nabla_x \phi_i (h(w^{(t)};i)) , \epsilon_i^{(t)} \rangle \\
%     %
%     & \overset{(a)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     & \quad + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + 2 \| h(w^{(t)};i) - h_i^* \| \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \| \\ & \quad - 2 \alpha_i^{(t)} \langle  h(w^{(t)};i) - h_i^* , \nabla_x \phi_i (h(w^{(t)};i)) \rangle + 2 \| h(w^{(t)};i) - h_i^* \| \| \epsilon_i^{(t)} \| \\
%     & \quad + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \\
%     & \quad + ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 + \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + \| \epsilon_i^{(t)} \|^2 \\
%     %
%     & \overset{\peqref{eq_phi_convex},\peqref{eq_ass_bounded_output}}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + 3 ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     & \quad + 3 ( \alpha_i^{(t)} )^2 \| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 + 3 \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + 2 D \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \| + 2 D \| \epsilon_i^{(t)} \| \\
%     & \quad - 2 \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] \\
%     %
%     & \overset{(b)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + 3 ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     & \quad + 3 \| \epsilon_i^{(t)} \|^2 + 2 D \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \| + 2 D \| \epsilon_i^{(t)} \| \\
%     & \quad - 2 ( 1 - 3 \alpha) \alpha_i^{(t)} [ \phi_i (h(w^{(t)};i)  ) - \phi_i (h_i^* ) ] \\
%     %
%     & \overset{(c)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + 3 ( \eta^{(t)} )^2 \| H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)})  \|^2 \\
%     & \quad + 3 \| \epsilon_i^{(t)} \|^2 + 2 D \| \eta^{(t)} H_i^{(t)} (v^{(t)} - v_{*\ \text{reg}}^{(t)}) \| + 2 D \| \epsilon_i^{(t)} \| \\
%     & \quad - \frac{( 1 - 3 \alpha)  \alpha}{L_{\phi}}  [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] \\
%     %
%     & \overset{(d)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 + 3 C^2 H^2 \| v^{(t)} - v_{*\ \text{reg}}^{(t)}  \|^2 + 3 \| \epsilon_i^{(t)} \|^2 \\
%     & \quad + 2 D C H  \| v^{(t)} - v_{*\ \text{reg}}^{(t)}  \|  + 2 D \| \epsilon_i^{(t)} \| - \frac{( 1 - 3 \alpha)  \alpha}{L_{\phi}}  [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] \\
%     %
%     & \overset{(e)}{\leq} \| h(w^{(t)};i) - h_i^* \|^2 - \frac{( 1 - 3 \alpha)  \alpha}{L_{\phi}}  [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ] \\
%     & \quad + 6 C^2 H^2 \varepsilon^2 + 3 c (4 \varepsilon^2 + 2 V)^2 G^2 C^4 \varepsilon^4 + 2 \sqrt{2} D C H \varepsilon \\ & \quad + 2 D \sqrt{c} (4 \varepsilon^2 + 2 V) G C^2 \varepsilon^2, 
% \end{align*}
% where $(a)$ follows by applying Young's inequality: $| \langle a , b \rangle | \leq \frac{\| a \|^2}{2} + \frac{\| b \|^2}{2}$ and Cauchy–Schwarz inequality $| \langle a, b \rangle | \leq \| a \| \| b \|$, $(b)$ follows by applying \peqref{eq_phi_convex_smooth} to get $\| \nabla_x \phi_i (h(w^{(t)};i)) \|^2 \leq 2 L_{\phi} [ \phi_i (h(w^{(t)};i)) - \phi_i (h_i^* ) ]$ and the fact that $\alpha_i^{(t)} \leq \frac{\alpha}{L_{\phi}}$, for some $\alpha \in (0, \frac{1}{3})$; $(c)$ follows by choosing $\alpha_i^{(t)} = \frac{\alpha}{2 L_{\phi}} \leq \frac{\alpha}{L_{\phi}}$; $(d)$ follows by using matrix vector inequality $\| H v \| \leq \| H \| \|v \| $, where $H \in \mathbb{R}^{c \times d}$ and $v \in \mathbb{R}^d$ \textbf{(NEED TO CHECK THIS since $H$ is non-square)} and Assumption~\ref{ass_bounded_hessian} in \peqref{eq_ass_bounded_hessian} and $\eta^{(t)} = C \sqrt{\varepsilon}$ for some $C > 0$ and $\varepsilon > 0$; $(e)$ follows by Lemmas~\ref{lem_bound_v} and \ref{lem_bound_epsilon}. 

% Rearranging the terms above, we have
% \begin{align*}
%      \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) & \leq \frac{L_{\phi}}{( 1 - 3 \alpha)  \alpha} [  \| h(w^{(t)};i) - h_i^* \|^2  -   \| h(w^{(t+1)};i) - h_i^* \|^2  ] \\
%     & \quad + \frac{6 C^2 H^2 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^2 + \frac{3 c (4 \varepsilon^2 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^4 \\ & \quad + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon + \frac{2 D \sqrt{c} (4 \varepsilon^2 + 2 V) G C^2 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^2
% \end{align*}

% Taking the average sum from $t = 0,\dots,T-1$, we have
% \begin{align*}
%      \frac{1}{T} \sum_{t=0}^{T-1}  [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  & \leq \frac{L_{\phi}}{( 1 - 3 \alpha)  \alpha T} \| h(w^{(0)};i) - h_i^* \|^2 \\
%     & \quad + \frac{6 C^2 H^2 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^2 + \frac{3 c (4 \varepsilon^2 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^4 \\ & \quad + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon + \frac{2 D \sqrt{c} (4 \varepsilon^2 + 2 V) G C^2 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^2
% \end{align*}

% Taking the average sum from $i = 1,\dots,n$, we have
% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  & \leq \frac{L_{\phi}}{( 1 - 3 \alpha)  \alpha T} \frac{1}{n} \sum_{i=1}^n \| h(w^{(0)};i) - h_i^* \|^2 \\
%     & \quad + \frac{6 C^2 H^2 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^2 + \frac{3 c (4 \varepsilon^2 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^4 \\ & \quad + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon + \frac{2 D \sqrt{c} (4 \varepsilon^2 + 2 V) G C^2 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^2. \tagthis \label{eq_average_phi_01}
% \end{align*}

% Note that
% \begin{align*}
%      \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ \phi_i (h(w^{(t)};i) ) - \phi_i (h_i^* ) ]  = \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ]. \tagthis \label{eq_average_phi_02}
% \end{align*}

% \begin{ass}\label{ass_diff_optimal_eps}
% For some $\delta > 0$, we have
% \begin{align*}
%     \Big | F_* - \frac{1}{n} \sum_{i=1}^{n} \phi_i (h_i^* )  \Big | \leq \delta. \tagthis \label{eq_ass_diff_optimal_eps}
% \end{align*}
% \end{ass}

% Hence, applying Assumption~\ref{ass_diff_optimal_eps} with $\delta = P \varepsilon$ for some $P > 0$ and $\varepsilon > 0$, we have
% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} [ F (w^{(t)}) - F_* ] & = \frac{1}{T} \sum_{t=0}^{T-1} \left( \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] - \left[ F_* - \frac{1}{n} \sum_{i=1}^{n} \phi_i (h_i^* )  \right] \right) \\
%     & \leq \frac{1}{T} \sum_{t=0}^{T-1} \frac{1}{n} \sum_{i=1}^n [ f (w^{(t)}; i) - \phi_i (h_i^* )  ] \\% + P \varepsilon \\
%     % 
%     & \overset{\peqref{eq_average_phi_01},\peqref{eq_average_phi_02}}{\leq} \frac{L_{\phi}}{( 1 - 3 \alpha)  \alpha T} \frac{1}{n} \sum_{i=1}^n \| h(w^{(0)};i) - h_i^* \|^2 \\
%     & \quad + \frac{6 C^2 H^2 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^2 + \frac{3 c (4 \varepsilon^2 + 2 V)^2 G^2 C^4 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^4 \\ & \quad + \frac{2 \sqrt{2} D C H L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon + \frac{2 D \sqrt{c} (4 \varepsilon^2 + 2 V) G C^2 L_{\phi}}{( 1 - 3 \alpha)  \alpha} \varepsilon^2 + P \varepsilon. 
% \end{align*}

% Then, we have
% \begin{align*}
%     \frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E} [ F (w^{(t)}) - F_* ] \leq \mathcal{O}(\varepsilon)
% \end{align*}

% after $T = \Ocal(\frac{1}{\varepsilon})$. Hence, the total complexity is $\mathcal{O}\left(\frac{n (C^2 H^2 + \varepsilon^2)}{\varepsilon^3} \log(1/\varepsilon^4) \right)$. \textbf{[It is possible to write explicitly]} 

% ======= OLD ANALYSIS (END) ===============





